Unsupervised Adversarially-Robust Representation Learning on Graphs

Unsupervised/self-supervised pre-training methods for graph representation learning have recently attracted increasing research interests, and they are shown to be able to generalize to various downstream applications. Yet, the adversarial robustness of such pre-trained graph learning models remains largely unexplored. More importantly, most existing defense techniques designed for end-to-end graph representation learning methods require pre-specified label definitions, and thus cannot be directly applied to the pre-training methods. In this paper, we propose an unsupervised defense technique to robustify pre-trained deep graph models, so that the perturbations on the input graph can be successfully identified and blocked before the model is applied to different downstream tasks. Specifically, we introduce a mutual information-based measure, \textit{graph representation vulnerability (GRV)}, to quantify the robustness of graph encoders on the representation space. We then formulate an optimization problem to learn the graph representation by carefully balancing the trade-off between the expressive power and the robustness (\emph{i.e.}, GRV) of the graph encoder. The discrete nature of graph topology and the joint space of graph data make the optimization problem intractable to solve. To handle the above difficulty and to reduce computational expense, we further relax the problem and thus provide an approximate solution. Additionally, we explore a provable connection between the robustness of the unsupervised graph encoder and that of models on downstream tasks. Extensive experiments demonstrate that even without access to labels and tasks, our model is still able to enhance robustness against adversarial attacks on three downstream tasks (node classification, link prediction, and community detection) by an average of +16.5% compared with existing methods.

==> Robust unsupervised representation learning on graphs/abstract.tex <==
%!TEX root = robustgraph.tex

\begin{abstract}
Unsupervised/self-supervised pre-training methods for graph representation learning have recently attracted increasing research interests, and they are shown to be able to generalize to various downstream applications. Yet, the adversarial robustness of such pre-trained graph learning models remains largely unexplored. More importantly, most existing defense techniques designed for end-to-end graph representation learning methods require pre-specified label definitions, and thus cannot be directly applied to the pre-training methods. In this paper, we propose an unsupervised defense technique to robustify pre-trained deep graph models, so that the perturbations on the input graph can be successfully identified and blocked before the model is applied to different downstream tasks. Specifically, we introduce a mutual information-based measure, \textit{graph representation vulnerability (GRV)}, to quantify the robustness of graph encoders on the representation space. We then formulate an optimization problem to learn the graph representation by carefully balancing the trade-off between the expressive power and the robustness (\emph{i.e.}, GRV) of the graph encoder. The discrete nature of graph topology and the joint space of graph data make the optimization problem intractable to solve. To handle the above difficulty and to reduce computational expense, we further relax the problem and thus provide an approximate solution. Additionally, we explore a provable connection between the robustness of the unsupervised graph encoder and that of models on downstream tasks. Extensive experiments demonstrate that even without access to labels and tasks, our model is still able to enhance robustness against adversarial attacks on three downstream tasks (node classification, link prediction, and community detection) by an average of +16.5\% compared with existing methods.

\end{abstract}

==> Robust unsupervised representation learning on graphs/conclusion.tex <==
%!TEX root = robustgraph.tex

\section{Conclusion}
In this paper, we study unsupervised adversarially robust representation learning on graphs. 
%focus on the problem of learning robust graph encoders on unlabeled data. 
We propose the graph representation vulnerability (GRV) to quantify the robustness of an unsupervised graph encoder. 
Then we formulate an optimization problem to study the trade-off between the expressive power of the encoder and its robustness to adversarial attacks. 
After that we propose an approximate solution 
which relies on a reduced empirical search space. 
We further build sound theoretical connections between GRV and one example downstream task, node classification.
Extensive experimental results demonstrate the effectiveness of our method on blocking perturbations on input graphs, sregardless of the downstream tasks.


==> Robust unsupervised representation learning on graphs/exp.tex <==
%!TEX root = robustgraph.tex

\section{Experiments} \label{sec:exp}
In this section, we demonstrate that our model capable of learning  highly-qualified representations that are robust to adversarial attacks.
In the experiments, we train our model in a fully unsupervised manner, then apply the output representations to three graph learning tasks: namely, node classification, link prediction, and community detection.
We demonstrate that compared with non-robust and other robust graph representation models, the proposed model produces robust representations to defend adversarial attacks (\S~\ref{sec:result-task}).
Furthermore, the superiority of our model still hold under different strengths of attacks (in \S\ref{sec:result-pert}) and under various attach strategies (\S\ref{sec:result-str}).

\begin{table*}[]
    % \small
	\centering
	\caption{Summary of results for the node classification, link prediction and community detection tasks using polluted data.}
	\vspace{-0.05in}
% \resizebox{\columnwidth}{!}{
% 	\setlength{\tabcolsep}{1pt}
	\begin{tabular}{l|ccc|ccc|ccc} \toprule
		& \multicolumn{3}{c|}{Node classification (Acc\%)} & \multicolumn{3}{c|}{Link prediction (AUC\%)} & \multicolumn{3}{c}{Community detection (NMI\%)} \\ \midrule
		{\diagbox [width=7em,trim=l] {Model}{Dataset}} &Cora &Citeseer &Polblogs &Cora &Citeseer &Polblogs &Cora &Citeseer &Polblogs \\ \midrule
		$\mathrm{Raw}$ &57.4$\pm$3.0 &49.7$\pm$1.6 &73.9$\pm$0.9 &60.5$\pm$0.1 &50.2$\pm$0.5 &89.0$\pm$0.4 &9.7$\pm$7.5  &1.0$\pm$0.5 &0.2$\pm$0.1\\
		$\mathrm{DeepWalk}$ &56.2$\pm$1.1 &16.5$\pm$0.9 &80.4$\pm$0.5 &55.4$\pm$0.8  &50.3$\pm$0.3  &89.2$\pm$0.7 &34.6$\pm$0.6 &11.1$\pm$1.0 &0.4$\pm$0.5 \\
		$\mathrm{DeepWalk}+\mathbf{X}$ &59.3$\pm$0.4 &26.5$\pm$0.5 &- &55.9$\pm$0.6 &50.9$\pm$0.3 &-  &34.2$\pm$3.7 &11.1$\pm$1.3 &-\\ 
		$\mathrm{GAE}$ &14.0$\pm$1.2 &16.2$\pm$1.1 &49.9$\pm$1.2  &52.4$\pm$1.4  &50.9$\pm$1.8 &50.5$\pm$1.3 &10.9$\pm$2.1  &1.4$\pm$1.7 &9.2$\pm$1.0 \\
		$\mathrm{DGI}$ &69.3$\pm$2.8 &53.2$\pm$2.2 &75.2$\pm$2.4 &68.6$\pm$0.4 &57.6$\pm$2.1 &91.2$\pm$1.1 &30.3$\pm$3.5  &8.5$\pm$3.8 &6.0$\pm$5.6 \\ \midrule
		$\mathrm{Dwns\_AdvT}$ &59.2$\pm$1.2 &25.0$\pm$1.0 &80.7$\pm$0.5 &56.0$\pm$0.7 &50.7$\pm$0.4 &89.5$\pm$0.8 &35.0$\pm$0.7 &11.5$\pm$1.0 &0.9$\pm$0.7\\
		$\mathrm{RSC}$ &46.9$\pm$3.5 &34.0$\pm$2.2 &58.9$\pm$1.7 &52.5$\pm$0.4 &57.2$\pm$0.2 &61.5$\pm$0.4 &4.9$\pm$0.7 &1.8$\pm$0.4 &4.4$\pm$4.3 \\
		$\mathrm{DGI}$-$\mathrm{EdgeDrop}$ &56.0$\pm$4.3 &49.0$\pm$4.5 &79.8$\pm$1.7  &66.2$\pm$0.8 &61.3$\pm$0.9  &89.3$\pm$1.6 &30.1$\pm$6.8  &7.34$\pm$0.8 &9.0$\pm$7.8\\
		$\mathrm{DGI}$-$\mathrm{Jaccard}$ &69.4$\pm$2.8 &57.1$\pm$1.3 &79.3$\pm$0.8 & 63.8$\pm$0.8  &57.6$\pm$1.0 & 84.7$\pm$0.9 &16.4$\pm$1.1  &6.1$\pm$0.6 &12.9$\pm$0.0\\
		$\mathrm{DGI}$-$\mathrm{SVD}$ &68.1$\pm$8.0 &56.1$\pm$16.4 &81.6$\pm$0.7 &60.1$\pm$0.8 &54.7$\pm$1.3 &85.2$\pm$0.7 &16.2$\pm$0.9  &6.5$\pm$0.8 &13.0$\pm$0.0\\ \midrule
		$\mathrm{Ours}$-$\mathrm{soft}$ &69.4$\pm$0.7 &57.5$\pm$2.0 &79.7$\pm$2.1 &68.1$\pm$0.3 &58.2$\pm$1.3 &90.3$\pm$0.5 &39.2$\pm$8.8  &23.5$\pm$1.9 &12.6$\pm$9.6\\
		$\mathrm{Ours}$ &\textbf{70.7$\pm$0.9} &\textbf{58.4}$\pm$1.4 &\textbf{82.7}$\pm$2.2 &\textbf{69.2}$\pm$0.4  &\textbf{59.8}$\pm$1.3 &\textbf{91.8}$\pm$0.4 &\textbf{41.4}$\pm$4.7 &\textbf{23.6}$\pm$2.8 &\textbf{14.8}$\pm$2.7 \\ \bottomrule
	\end{tabular}
	\label{tab:main}
	\vspace{-0.05in}
\end{table*}

\subsection{Experimental Setup}\label{sec:setup}
\vpara{Datasets.}
We conduct experiments on three benchmark datasets: Cora, Citeseer
% ~\cite{sen:aimag08} 
and  Polblogs.
% ~\cite{adamic2005political}. 
The first two of these are well-known citation networks  in which nodes are documents and edges are the citation links between two documents. Polblogs is a network of US politics weblogs, where nodes are blogs and the connection between two blogs forms an edge. As Polblogs is a dataset without node attributes, the identity matrix is used to create its node attributes.

\vpara{Baselines.}
The baseline models roughly fall into two categories.
\begin{itemize}[leftmargin=*]
\item \textbf{Non-robust graph representation learning}:
1) Raw: raw features concatenating the graph topology and the node attributes (graph topology (only) for Polblogs);
2) DeepWalk~\cite{perozzi2014deepwalk}: a random walk-based unsupervised representation learning method that only considers the graph topology;
3) DeepWalk+X: concatenating the Deepwalk embedding and the node attributes; 
4) GAE~\cite{kipf2016variational}: variational graph auto-encoder, an unsupervised representation learning method; and
5) DGI~\cite{velickovic2018deep}: another unsupervised representation learning method based on MI.

\item \textbf{Defense models}:
1) Dwns\_AdvT~\cite{10.1145/3308558.3313445}: a defense model designed for Deepwalk; 
2) RSC~\cite{bojchevski2017robust}: a robust unsupervised representation learning method via spectral clustering;
3) DGI-EdgeDrop~\cite{Rong2020DropEdge}: a defense model that works by dropping 10\% of edges during training DGI;
4) DGI-Jaccard~\cite{wu2019adversarial}: DGI applied to a pruned adjacency matrix in which nodes with low Jaccard similarity are forced to be disconnected; and
5) DGI-SVD~\cite{entezari2020all}: DGI applied to a low-rank approximation of the adjacency matrix obtained by truncated SVD.
\end{itemize}
We also include Ours-soft, an variant of our model which removes soft margin on GRV.

\vpara{Implementation details.}
In the training phase, we adopt the graph PGD attack to construct adversarial examples of $\boldsymbol{a}$ while the PGD attack~\cite{madry2017towards} to construct adversarial examples of~$\boldsymbol{x}$.
We set the hyperparameters $\gamma=5\mathrm e\text{-}3$, $\delta=0.4|\mathbf E|$, and $\epsilon=0.1$.
For Polblogs, we do not perform attacks on the constructed node attributes.

In evaluation, we use the same attack strategy as in the training phase. 
Note that DeepWalk and RSC both require the entire graph, 
%to learn the node embedding, 
and thus we have to retrain them using polluted data.
Due to the imperceptible constraint on adversarial attacks, we set $\delta=0.2|\mathbf E|$ during evaluation.
The evaluation is performed on three downstream tasks, and we explain the detailed settings below.
\begin{itemize}[leftmargin=*]
\item Node classification: logistic regression is used for evaluation, and only accuracy score is reported as the test sets are almost balanced. 
For Cora and Citeseer, we use the same dataset splits as in~\cite{kipf2017semi}, but do not utilize the labels in the validation set. For Polblogs, we allocate 10\% of the data for training and 80\% for testing.

\item Link prediction: logistic regression is used to predict whether a link exists or not.
Following conventions,  we generate the positive test set by randomly removing 10\% of existing links and form the negative test set by randomly sampling the same number of nonexistent links. The training set consists of the remaining 90\% of existing links and the same number of additionally sampled nonexistent links. We use the area under the curve (AUC) as the evaluation metric on the link prediction task.

\item Community detection: following the basic schemes for community detection based on graph representation learning, we apply the learned representations to the K-means algorithm. The normalized mutual information (NMI) is used as the evaluation metric here.
\end{itemize}
We run 10 trials for all the experiments and report the average performance and standard deviation.

\subsection{Performance on Downstream Tasks} \label{sec:result-task}

After adversarial attacks on graph topology and node attributes, our model's performance drops by an average of 13.6\%, 1.0\% and 47.3\% on the node classification, link prediction and community detection task, respectively. 
It's worth noting that, in community detection, adversarial attacks can cause dramatic influence on model performance because the community detection task itself is very sensitive to the graph topology.
Table~\ref{tab:main} summarizes the performance of different models in three downstream tasks.
From the table we see that our model beats the best baseline by an average of +1.8\% on the node classification task, +1.8\% on the link prediction task and +45.8\% on the community detection task.
The difference between the performance of our model and that of those non-robust graph learning models indicates the importance of defending adversarial attacks.
Moreover, our model still stands out with huge lead when compared with existing defense models.
Last but not least, the ablation study, \emph{i.e.}, comparing the last two rows in Table~\ref{tab:main}, shows the superiority of the soft margin on GRV.
With this penalty, the model focuses on the representation capability on clean data when the encoder is robust enough (\emph{i.e.}, $\mathrm{RV}_\tau \leq \gamma$), while carefully balances the trade-off between the performance on clean data and the robustness to polluted ones.

\begin{figure}[t]
\centering
	\includegraphics[width=0.5\textwidth]{fig/attack.pdf}\\
% \includegraphics[width=0.236\textwidth]{fig/a_attack.pdf}
% % \hspace{0.01\textwidth}
% \includegraphics[width=0.236\textwidth]{fig/e_attack.pdf}
% 	\captionsetup[subfigure]{labelformat=simple}
% 	\centering  
% 	\subfloat[Accuracy under different perturbation rate $\delta$]{
% 		\parbox{.23\textwidth}{
% 			\centering
% 			\includegraphics[width=0.2\textwidth]{fig/a_attack.pdf}
% 		}
% 	}
% 	\subfloat[Accuracy under different perturbation rate $\epsilon$]{
% 		\parbox{.23\textwidth}{
% 			\centering
% 			\includegraphics[width=0.2\textwidth]{fig/e_attack.pdf}
% 		}
% 	}
\caption{Accuracy of different models under various perturbation rates $\delta$ and $\epsilon$. The downstream task is node classification and we use the Cora dataset for illustration. The shaded area indicates the standard deviation ($\times 0.1$) over 10 runs.}
\vspace{-0.05in}
\label{fig:robust}
\end{figure} 

\subsection{Performance under Different Rates of Perturbation} \label{sec:result-pert}

We further compare our model with several strong competitors under various perturbation rates.
We use the node classification task and the Cora dataset as an illustrative example.
We vary the strength of adversarial attacks on the graph topology and the node attributes by choosing different perburation rates $\delta$ and $\epsilon$, respectively.
As shown in Figure~\ref{fig:robust}, the performance of our model is consistently superior to other competitors, both on average and in worst-case.
Note that the strong competitor DGI generates negative samples in the training phase,
and this might explain the robustness of the DGI model.
Comparably, the high standard deviation of DGI-SVD might be attributed to the continuous low-rank approximation of the adjacency matrix: the output of truncated SVD is no longer a 0--1 matrix, which violates the discrete nature of graph topology.

\begin{table}[t]	
	\centering
	\caption{Defense against different attackers on Polblogs for the node classification task.}
	\vspace{-0.05in}
% 	\setlength{\arraycolsep}{1pt}
	\begin{tabular}{lcccc}
		\toprule
		{\diagbox [width=7em,trim=l] {Model}{Attacker}}  &$\mathrm{Degree}$ &$\mathrm{Betw}$ &$\mathrm{Eigen}$  & $\mathrm{DW}$  \\ \midrule
		$\mathrm{Raw}$ &87.4$\pm$0.3 &84.1$\pm$0.8 &86.4$\pm$0.6 &87.9$\pm$0.4 \\
		$\mathrm{DeepWalk}$ &87.8$\pm$0.9 &83.5$\pm$1.2 &84.3$\pm$1.0 &87.7$\pm$0.9 \\
		$\mathrm{DeepWalk}+\mathbf{X}$ &85.8$\pm$2.7 &82.7$\pm$2.1 &85.0$\pm$1.1 &88.3$\pm$0.9 \\ 
		$\mathrm{GAE}$  &83.7$\pm$0.9 &81.0$\pm$1.6 &81.5$\pm$1.4 &85.4$\pm$1.1 \\
		$\mathrm{DGI}$  &86.6$\pm$1.1 &84.8$\pm$1.2 &84.8$\pm$1.0  &86.4$\pm$1.1    \\
		\hline   
		$\mathrm{Dwns\_AdvT}$ &88.0$\pm$1.0 &84.1$\pm$1.3 &84.6$\pm$1.0 &88.0$\pm$0.8 \\
		$\mathrm{RSC}$  &52.1$\pm$1.3 &51.9$\pm$0.7 &51.4$\pm$0.5 &52.6$\pm$1.1 \\
		$\mathrm{DGI}$-$\mathrm{EdgeDrop}$ &87.1$\pm$0.3 &\textbf{87.0}$\pm$0.6 &80.5$\pm$0.5 &86.3$\pm$0.3 \\
		$\mathrm{DGI}$-$\mathrm{Jaccard}$ &82.1$\pm$0.3 &80.7$\pm$0.4 &80.6$\pm$0.3 &82.2$\pm$0.2 \\
		$\mathrm{DGI}$-$\mathrm{SVD}$ &86.5$\pm$0.2 &85.6$\pm$0.2 &86.1$\pm$0.2 &85.3$\pm$0.3 \\
		\hline
		$\mathrm{Ours}$-$\mathrm{soft}$ &88.5$\pm$0.7 &85.7$\pm$1.5 &86.2$\pm$0.4 &88.7$\pm$0.7 \\
		$\mathrm{Ours}$ &\textbf{89.3}$\pm$0.7 &86.3$\pm$1.2 &\textbf{86.7}$\pm$0.4 &\textbf{89.0}$\pm$0.8  \\
		\bottomrule
	\end{tabular}
	\vspace{-0.08in}
	\label{tab:transfer}
\end{table}

\subsection{Performance under Other Attack Strategies} \label{sec:result-str}

In practice we do not know which kind of attack strategies the malicious users is going to use.
Thus it is interesting and important to know the performance of our model across different types of adversarial attacks.
We adapt some common attack strategies to the unsupervised setting and use them as baselines.
1) Degree: flip edges based on the sum of the degree centrality of two end nodes;
2) Betw: flip edges based on the sum of the betweenness centrality of two end nodes;
3) Eigen: flip edges based on the sum of the eigenvector centrality of two end nodes; and 
4) DW~\cite{bojchevski2019adversarial}: a black-box attack method designed for DeepWalk. We set the size of the sampled candidate set to 20K, as suggested in ~\cite{bojchevski2019adversarial}. 

This time we consider the node classification task on Polblogs dataset for illustration.
This choice is convincing because all the above attack strategies only vary the graph topology, which is the only information we know about Polblogs dataset.
Results in Table~\ref{tab:transfer} shows the outstanding performance of our model as its superiority persists in three attack strategies out of four.
Comparison between Table~\ref{tab:main} and Table~\ref{tab:transfer} shows that the graph PGD attack via MI is the most effective attack strategy used here.
This observation verifies the idea of our model: We learn from the worst adversarial example (\emph{i.e.}, the one deteriorates the performance most).


==> Robust unsupervised representation learning on graphs/impact.tex <==
%!TEX root = robustgraph.tex

\section{Ethics Statement}
\label{sec:impact}

Recently, deep learning on graphs has shown excellent results in different real-world applications including molecule analysis~\cite{hamilton2017inductive}, drug discovery~\cite{gilmer2017neural}, financial surveillance~\cite{paranjape2017motifs}, recommendation systems~\cite{wang2019knowledgeaware}, \emph{etc.}
Despite these impressive results, the research community has recently shown that graph learning models are vulnerable to adversarial attacks~\cite{chen2020survey, bojchevski2019adversarial, zugner2019adversarial}.
A graph attacker can intentionally modify the original graph such that the modifications are almost human-imperceptible, which can cause wrong predictions in graph learning models. The real-life applications of such attacks can be very serious, for instance, one could create some false connections with rich people to increase his/her credit score in an online payment company, then he/she will be able to get loan and run away from the system. 
For that reason, there is a pressing need to learn robust representations on graphs against these adversarial attacks.

In this paper, we focus on the underlying problem of learning robust representations via mutual information on graphs and further establish a theoretical connection between our robustness measure and the robustness of downstream classifiers. Our approach and analysis provide us some novel perspectives to better understand the vulnerability of graph learning models when facing with graph adversarial attacks.
Accordingly, we think our technology can bring beneficial impacts to the society. We would also encourage further works to develop better defense methods to maintain a more robust learning environment.

==> Robust unsupervised representation learning on graphs/intro.tex <==
%!TEX root = robustgraph.tex

\section{Introduction} \label{sec:intro}

\begin{figure}[t]  
	\centering  
	\includegraphics[width=0.5\textwidth]{fig/introfinal.pdf}\\
	\caption{Overview of a graph pre-training pipeline under adversarial attacks. 
	If the graph encoder is vulnerable to the attacks, the adversarial risk would propagate to every downstream task via the perturbed graph representation.
	}
	\vspace{-0.08in}
	\label{fig:intro}     
\end{figure}  

% background: importance of graphs; goal of graph representation learning; mention our application scenarios. 
Graphs, a common mathematical abstraction for modeling pairwise interactions between objects, are widely applied in numerous domains, including bioinformatics, social networks, chemistry, and finance.
Owing to their prevalence, deep learning on graphs, such as graph neural networks (GNNs)~\cite{kipf2017semi,hamilton2017inductive}, have recently undergone rapid development, making major progress in various analytical tasks, including node classification~\cite{kipf2017semi, hamilton2017inductive}, link prediction~\cite{kipf2016variational}, and graph classification~\cite{xu2018how}. However, most deep learning models on graphs are trained with task-specific labels in an end-to-end manner for a particular task. This motivates some recent efforts to pre-train an expressive graph encoder on unlabeled data and further feed the learned representations to (supervised/unsupervised) off-the-shelf machine learning models for relevant downstream tasks~\cite{hu2019strategies, hu2020gpt, qiu2020gcc}. 
% The graph representations learned by pre-training models are directly applicable to various downstream tasks with a simple and inexpensive machine learning model attached after the encoded representations.
The pre-training models on graphs enable the learned representations to be directly applicable to different applications with a simple and inexpensive machine learning model attached after the encoded representations.

Despite the promising results achieved by deep learning models on graphs, recent studies have shown that these models are vulnerable to adversarial attacks~\cite{dai2018adversarial, zugner2019adversarial, bojchevski2019adversarial}. In other words, even imperceptible perturbations on graph topology and node attributes can significantly affect the learned graph representation, thereby degrading the performance of downstream tasks~\cite{chen2020survey}. This so-called adversarial vulnerability has given rise to tremendous concerns regarding the utilization of deep learning models on graphs, especially in security-critical applications such as drug discovery~\cite{gilmer2017neural} and financial surveillance~\cite{paranjape2017motifs}.
However, the adversarial vulnerability of pre-training models on graphs is far overlooked.
In this work, we show that graph pre-training models also suffer from the adversarial vulnerability problem. 
Actually, owing to the complicated and deep structure, the graph encoder is more vulnerable to adversarial attacks than the simple machine learning models used for downstream tasks in a graph pre-training pipeline~\cite{tanay2016boundary}. 
As Figure~\ref{fig:intro} shows, once the graph encoder is vulnerable to adversarial attacks, the adversarial risk would propagate to every downstream task via the perturbed representations. 

Most efforts targeted on this adversarial vulnerability problem focus on supervised, end-to-end models designed for a particular application scenario~\cite{zugner2019certifiable, bojchevski2019certifiable, wang2019graphdefense, jin2020graph}.
However, the dependency on the supervised information largely limits the scope of their application and usefulness.
For example, these models do not perform well on downstream tasks in which training labels are missing, \emph{e.g.}, community detection in social networks.
In addition, training multiple models for different downstream tasks is both costly and insecure~\cite{feurer5872efficient}.
In contrast, robust unsupervised pre-training models can easily handle the above issues: adversarial attacks are identified and blocked before propagating to downstream tasks.
Moreover, these models are applicable to a more diverse group of applications, including node classification, link prediction, and community detection.
%To the best of our knowledge, 
And yet, robust pre-training models under the unsupervised setting remains largely unexplored. 
%is still a new research area.

There are many interesting yet challenging questions in this new field of research. 
Conventionally, the robustness of a model is defined based on the label space~\cite{hao2020adversarial, zugner2019certifiable, bojchevski2019certifiable}, which is not the case in our setting.
Thus the first difficulty we meet is to quantify the robustness of an unsupervised model (without the knowledge of the true or predicted labels).

To overcome the above challenge, in this paper, we first introduce the \emph{graph representation vulnerability} (GRV), an information theoretic-based measure used to quantify the robustness of a graph encoder. We then formulate an optimization problem to study the trade-off between the expressive power of a graph encoder and its robustness to adversarial attacks, measured in GRV.
However, how to efficiently compute or approximate the objective of the optimization problem becomes the next issue.
First, it remains a big problem on how to describe the ability of the attack strategies or the boundary of perturbations, because adversarial attacks on graphs perturb both the discrete graph topology and the continuous node attributes. 
Second, the rigorous definition of the objective 
% involving the MI and the adversarial distribution 
is intractable.
% but also raises computational bottleneck.
% \JR{directly computing the objective is nontrivial because estimating the MI and the joint adversarial distribution w.r.t discrete graph topology and continuous node attributes is intractable, leading to the second challenge. }
% \XJ{Even when the robustness is well defined, how to efficiently compute or approximate this value becomes the next issue. In addition, adversarial attacks on graphs perturb both the discrete graph topology and the continuous node attributes.  Thus it remains a big problem on how to describe the ability of the attack strategies or the boundary of perturbations. Then, with the rigorous definition, a similar computational bottleneck arises again. Finally, even when the above-mentioned difficulties are resolved, we still need to solve an intractable optimization problem to find a highly-qualified, robust graph representation.}

To handle the above issues, we first quantify the ability of adversarial attacks using Wasserstein distance between probability distributions, and provide a computationally efficient approximation for it. We then adopt a variant of projected gradient descent method to solve the proposed optimization problem efficiently. A sub-optimal solution for the problem gives us a well-qualified, robust graph representation encoder.
% further reduce the input search space to a more practical and explainable boundary, subsequently adopting a gradient-based method to efficiently find solutions in the discrete input space. 
% \XJ{ We quantify the ability of adversarial attacks using Wasserstein distance between probability distributions, and provide a computationally efficient approximation for it. We adopt a variant of projected gradient descent method to solve the proposed optimization problem efficiently. A sub-optimal solution for the problem gives us a well-qualified, robust graph representation encoder.}

Last but not least, we explore several interesting theoretical connections between the proposed measure of robustness (GRV) and the classifier robustness based on the label space.
To show the practical usefulness of the proposed model, we apply the learned representations to three different downstream tasks, namely, node classification, link prediction, and community detection. Experimental results reveal that under adversarial attacks, our model beats the best baseline by an average of +1.8\%, +1.8\%, and +45.8\% on node classification, link prediction, and community detection task, respectively. 
%\YS{even the baseline that relies on the knowledge of the task and labels?}


% In this paper, we propose a mutual information-based defense technique for graph pre-training models. We opt to directly robustify the unsupervised graph encoder because making the pretrained representation robust will significantly enhance the robustness of the whole pipeline.
% % we study the robustness of the unsupervised graph encoder so that the learned representations can be further feed to off-the-shelf machine learning models for different application scenarios. 
% This problem is nontrivial, and several related challenges remain. Conventionally, model robustness is often measured based on the label space~\cite{hao2020adversarial, zugner2019certifiable, bojchevski2019certifiable} --- in other words, we consider a model to be robust if its predictions over the label space are insensitive to input perturbation. So how to measure the model robustness without labels?
% %This is the first challenge we meet in this work. 
% %\YS{can you please summarize the challenges in (1) and (2)? Later sections refer there are first and second challenge, but I am not sure what they are referring to exactly.}

% % We propose a mutual-information based defense technique for pretrained deep graph models. Intuition about why it works: 1) the downstream classifiers are usually simple, so making the pretrained representation robust will significantly enhance the robustness of the whole pipeline; 2) the mutual information captures ... so it can serve as a good measure of robustness (for this one I'm not sure).
% To overcome the above challenge, in this paper, 
% we first introduce an information theoretic-based measure, \textit{graph representation vulnerability (GRV)}, to quantify the robustness of graph encoders under adversarial attacks both on the graph topology and node attributes. 
% Based on the GRV, we aim to learn the robust graph representation by trading off between the robustness and the expressive power of the encoder in the objective of the mutual information (MI) maximization principle.  However, directly computing the objective is nontrivial because estimating the MI and the joint adversarial distribution w.r.t discrete graph topology and continuous node attributes is intractable, leading to the second challenge. 

% \hide{Moreover, adding perturbations on both spaces $\mathcal{A}$ and $\mathcal{X}$ will make the robustness even more difficult to enhance,  -- unlike the image domain, where the instances are assumed to be i.i.d., while the adversarial perturbations of edges or node attributes can be easily propagated to other neighbors via the graph edges. }

% To handle the intractable problem, we 
% % first relax our problem to a constrained saddle point optimization problem. Then, we 
% further reduce the input search space to a more practical and explainable boundary, subsequently adopting a gradient-based method to efficiently find solutions in the discrete input space. 
% % \yang{check} 
% % \yang{Describe theoretical contribution}

% Last but not least, we explore several interesting theoretical connections between our proposed robustness measure GRV (which relies on the representation space) and the downstream classifiers (built on the label space) on graphs under certain assumptions. We further empirically demonstrate the practicality and generality of our approach by applying the learned representation to three different downstream tasks: node classification, link prediction, and community detection when no the knowledge of the tasks and task-specific labels is accessible. 
% % \YS{when no knowledge?}
% Experimental results demonstrate that under adversarial attacks, our model beats the best baseline by an average of +1.8\%, +1.8\%, and +45.8\% on node classification, link prediction, and community detection task, respectively. 
% \YS{even the baseline that relies on the knowledge of the task and labels?}
% % on node classification task, +1.8\% on link prediction task and +48.7\% on community detection under adversarial attacks.

\hide{
The rest of the paper is organized as follows.
In \S\ref{sec:pre} we present some useful notations.
Then in \S\ref{sec:model} we introduce the graph representation vulnerability (GRV) to quantify the robustness of graph encoder, formulate an optimization problem to explore the trade-off between the expressive power and the robustness of the graph encoder, and provide a sub-optimal solution to the problem.
We also illustrate the theoretical connection between GRV and the label space in \S\ref{sec:theory}.
Numerical experiments in \S\ref{sec:exp} demonstrate the robustness of our proposed method against adversarial attacks on graphs.
}

==> Robust unsupervised representation learning on graphs/model.tex <==
%!TEX root = robustgraph.tex

\section{Graphs Representations Robust to Adversarial Attacks} \label{sec:model}

In a widely adopted two-phase graph learning pipeline, The first step is to pre-train a graph encoder $e$ (without the knowledge of true labels), which maps the joint input space $\mathcal{S}$ (\emph{i.e.},  the graph topology~$\mathcal A$ and node attributes $\mathcal X$) into some, usually lower-dimensional, representation space $\mathcal{Z}$.
Then the encoded representation is used to solve some target downstream tasks.

In this section, we explain how to obtain a well-qualified graph representation robust to adversarial attacks.
We first propose a measure to quantify the robustness without label information in \S\ref{subsec:rv}.
In~\S\ref{subsec:opt}, we formulate an optimization problem to explore the trade-off between the expressive power and the robustness of the graph encoder.
We then describe every component in the proposed optimization problem, and explain how we obtain a sub-optimal solution efficiently in~\S\ref{subsec:solution}.

\subsection{Quantifying the Robustness of Graph Representations} \label{subsec:rv}

In this section, we propose the \emph{graph representation vulnerability} (GRV) to quantify the robustness of an encoded graph representation.
Intuitively, the learned graph representation is robust if its quality does not deteriorate too much under adversarial attacks.
Now we introduce in detail how to measure the quality of representations using MI, and how to describe the difference of representation quality before and after adversarial attacks.

% We propose a measure, \textit{graph representation vulnerability} (GRV), 
% from an information theoretic point of view. 
% %To fairly quantify the representation robustness, it is critical to understand the essence for the graph encoder to achieve high-quality representations. 
% %We first motivate the use of the mutual information between representation's input and output as our unsupervised representation learning objective. 
% %(see \textit{The use of the mutual information} section).
% The intuition behind GRV is: 
% the representations learned by a graph encoder are considered to be robust, 
% if its quality would not drop as much even under adversarial attacks in the worst-case.  
% Before introduce more details, we first motivate the use of the mutual information as the cornerstone of our measure. 
%if an attacker can decrease the quality of representations by a large margin, the representations learned by graph encoder are considered to be vulnerable to adversarial attacks. 
%Based on this intuition, we then introduce a robustness measure, graph representation vulnerability (GRV), 
% to the worst-case margin 
%for use in quantifying the robustness of graph representations.
%(see \textit{Graph representation vulnerability} section).

% In particular, it is critical to assess their vulnerability to adversarial attacks –
% To fairly quantify the representation robustness, we aim to address the following issues in a top-down fashion. First, considering that unsupervised learning of graph encoder $e$ seems ill-posed as there is no natural objective one should optimize, we start with an insight to measure the expressive power of graph encoder from an information theoretic point of view. Second, to better explore the adversarially-robust graph representations, we study the key mechanism of adversarial attacks that can hurt the graph representations most. Empowered with the above two points, we propose the \textit{graph representation vulnerability (GRV)} to quantify the robustness of the representations learned by graph encoder.

\vpara{The use of mutual information.} 
A fundamental challenge to achieving a qualified graph representation is the need to find a suitable objective that guides the learning process of the graph encoder. 
In the case of unsupervised graph representation learning, the commonly used objectives are random walk-based~\cite{perozzi2014deepwalk, grover2016node2vec} or reconstruction-based~\cite{kipf2016variational}. 
These objectives impose an inductive bias that neighboring nodes or nodes with similar attributes have similar representations. 
However, the inductive bias is easy to break under adversarial attacks~\cite{jin2020graph, entezari2020all}, leading to the vulnerability of random walk-based and reconstruction-based encoders. 
As an alternative solution, we turn to maximize the MI between the input attributed graph and the representation output by the encoder, \emph{i.e.}, $\mathrm I(S ; e(S))$.
In our case, maximizing the MI $\mathrm I(S; e(S))$ encourages the representations to be maximally informative about the input graph and to avoid the above-mentioned inductive bias.
% Therefore, the mutual information $\mathrm I(S; e(S))$ is a meaningful and useful measure of the encoded graph representation, and has achieved great success in learning well-qualified graph representations in an unsupervised manner~\cite{velickovic2018deep, sun2019infograph}.

\vpara{Graph representation vulnerability.}
In addition to the measure of the quality of a graph representation, we also need to describe the robustness of a representation.
% Before that, we are supposed to quantify the ability of the adversarial attacks.
% An attack strategy is viewed as a perturbed probability distribution around that of $S=(A,X)$, and then all possible attack strategies stay in a ball around the genuine distribution~$\mu_S$:
% \[
%     \mathcal B_\infty(\mu_S, \tau) = \{\mu_{S^\prime} \in \mathcal M(S) \colon W_\infty (\mu_S, \mu_{S^\prime}) \leq \tau\},
% \]
% where $W_\infty$ is the $\infty$-Wasserstein distance, and $\tau > 0$ is a pre-defined budget.
% Formally, the $p$-th Wasserstein distance between two probability measures $\mu_S$ and $\mu_{S^\prime}$ in a metric space $(\mathcal S, d)$ is defined as
% \[
%     W_p = (\mu_S, \mu_{S^\prime}) = \left( \inf_{\pi \in \Pi (\mu_S, \mu_{S^\prime})} \int_{\mathcal S^2} d(\boldsymbol s, \boldsymbol s^\prime) \, d\pi(\boldsymbol s, \boldsymbol s^\prime) \right)^{1/p},
% \]
% where $\Pi(\mu_S, \mu_{S^\prime})$ denotes the collection of all measures on $\mathcal S \times \mathcal S$ with marginal $\mu_S$ and $\mu_{S^\prime}$, respectively.
% The choice of $\infty$-Wasserstein distance (\emph{i.e.}, $p=\infty$) is conventional in learning graph representations~\cite{champion2008wasserstein}. \XJ{add citation}
Intuitively, an encoder is robust if the MI before and after the attack stay close enough.
Thus, we propose the \emph{graph representation vulnerability (GRV)} to quantify this difference:
\begin{equation} \label{eq:grv}
    \mathrm{GRV}_\tau (e) = \mathrm I (S; e(S)) - \inf_{\mu_{S^\prime} \in \mathcal B(\mu_S, \tau)} \mathrm I(S^\prime; e(S^\prime)),
\end{equation}
where $S=(A,X)$ is the random variable following the benign data distribution, and $S^\prime=(A^\prime, X^\prime)$ follows the adversarial distribution.
The first term $\mathrm I(S;e(S))$ in~\eqref{eq:grv} is the MI between the benign graph data and the encoded representation, while the term $\mathrm I(S^\prime, e(S^\prime))$ uses the graph data after attack.
The attack strategy~$\mu_{S^\star}$ that results in the minimum MI is called the \emph{worst-case} attack, and is defined as
\[
    \mu_{S^\star} = \mathop{\rm argmin}_{\mu_{S^\prime} \in \mathcal B(\mu_S, \tau)} \mathrm I(S^\prime; e(S^\prime)).
\]
Hence by definition, the graph representation vulnerability (GRV) describes the difference of the encoder's behavior using benign data and under the worst-case adversarial attack.
A lower value of $\mathrm{GRV}_\tau(e)$ implies a more robust encoder to adversarial attacks. Formally, an encoder is called $(\tau, \gamma)$-robust if $\mathrm{GRV}_\tau(e) \leq \gamma$.

An analogy to the graph representation vulnerability (GRV) has been studied in the image domain~\cite{Zhu2020LearningAR}. However, the extension of~\cite{Zhu2020LearningAR} to the graph domain requires nontrivial effort. An image is considered to be a single continuous space while a graph is a joint space $\mathcal S=(\mathcal A, \mathcal X)$, consisting of a discrete graph-structure space $\mathcal A$ and a continuous feature space $\mathcal X$. 
Moreover, the perturbations on the joint space $(\mathcal A, \mathcal X)$ is difficult to track because a minor change in the graph topology or node attributes will propagate to other parts of the graph via edges.
This is different in the image domain, where the distributions of all the pixels are assumed to be i.i.d.
Therefore, the discrete nature of graph topology and joint space $(\mathcal A, \mathcal X)$ make the worst-case adversarial attack extremely difficult to estimate. Thus, the optimization method we apply is substantially different from that in~\cite{Zhu2020LearningAR}; see \S\ref{subsec:opt} and \S\ref{subsec:solution}.  Furthermore, more complicated analysis is needed to verify our approach in theory; see \S\ref{sec:theory} for details.
\hide{First, an image is considered to be a single continuous space while a graph is a joint space $\mathcal S=(\mathcal A, \mathcal X)$, consisting of a discrete graph-structure space $\mathcal A$ and a continuous feature space $\mathcal X$. The discrete nature of graph topology makes the worst-case adversarial attack extremely difficult to estimate. Thus, the optimization method we apply is substantially different from that in~\cite{Zhu2020LearningAR}; see \S\ref{subsec:opt} and \S\ref{subsec:solution}. 
Furthermore, in an image, the distribution which every pixel lies in is considered to be i.i.d. in~\cite{Zhu2020LearningAR}, which is not true in the graph domain. 
Thereby in our paper, more complicated analysis is needed to verify our approach in theory; see \S\ref{sec:theory} for details.}

% To further ensure that the graph encoder can function well under adversarial attacks, it is critical to reason about the attacker's % most harmful
% behavior.
% % in the worst case (\emph{i.e.}, the graph representations are damaged by the most threathing attack)
% % the attack does greatest harm to the graph representations).
% We first generally define various graph adversarial attack strategies as a set of adversarial distributions in a $\infty$-Wasserstein perturbation bound w.r.t $\mu_{S}$ as follows:
% \begin{linenomath}
% \begin{equation*}
%     \mathcal{B}_{\infty}(\mu_{S}, \tau)=\{\mu_{S^{\prime}} \in \mathcal{M}(\mathcal{S}): W_{\infty}(\mu_{S}, \mu_{S^{\prime}}) \le \tau \},
% \end{equation*}
% \end{linenomath}
% where $\mu_{S^{\prime}}$ is the adversarial distribution that one attack strategy follows, and
% the budget $\tau$ is to ensure that the attacker can not modify the graph completely.

% Given the set of adversarial distributions, we aim to figure out the worst-case adversarial distribution, \emph{i.e.}, the adversarial distribution that the most threatening attack strategy follows such that the mutual information between the perturbed representation's input and output is minimal.
% % , namely the \textit{worst-case adversarial distribution}.  
% We assume that any representations learned by the graph encoder are robust as long as the representations perturbed by the worst-case attack are robust.

% % Following the MI-based graph encoder, we naturally assume that the worst-case adversarial distribution is the one following which the attacker can minimize the mutual information between the perturbed representation's input and output, \emph{i.e.}, $\inf_{\mu_{S^{\prime}} \sim \mathcal{B}_{\infty}(\mu_{S}, \tau)} \mathrm{I}\left(S^{\prime} ; e\left(S^{\prime}\right)\right)$. 

% Accordingly, we consider that if the graph encoder is sufficiently robust, the 
% margin w.r.t the mutual information 
% before and after a worst-case attack would be small. 
% % before and after the worst-case adversarial attack would be small. 
% We therefore define the graph representation vulnerability (GRV) to quantify the representation robustness as:
% \begin{linenomath}
% \begin{align}
% &\text{GRV}_{\tau}(e) = \mathrm{I}\left(S ; e\left(S\right)\right) - \inf_{\mu_{S^{\prime}} \sim \mathcal{B}_{\infty}(\mu_{S}, \tau)}  \mathrm{I}\left(S^{\prime} ; e\left(S^{\prime}\right)\right) \\
% & \text{where} \ S = (A,X) \ \text{and}  \  S^{\prime}=(A^{\prime},X^{\prime}), \nonumber
% \end{align}
% \end{linenomath}
% \noindent where the \yang{infimum is attained to learn robust representations under the worst-case adversarial risk}, $S$ is the random variable following the benign data distribution, while $S^{\prime}$ denotes the variable following the adversarial distribution. A lower value of $\text{GRV}_{\tau}(e)$ implies that the graph encoder is more robust to the perturbations of input data distribution. Formally, a representation is deemed $(\tau, \gamma)$-robust if $\text{GRV}_{\tau}(e) \le \gamma$. 

% A similar concept related to the MI-based robustness measure is also discussed and adopted in the image domain~\cite{Zhu2020LearningAR}, in which only a single input space (\yang{\emph{i.e.}, the space of images}) is taken into consideration. 
% Instead, our proposed graph representation vulnerability is built upon a joint input space  $\mathcal{S}=(\mathcal{A}, \mathcal{X})$, consisting of one discrete graph-structure space $\mathcal{A}$ and one continuous feature space $\mathcal{X}$. 
% Meanwhile, unlike continuous input in the image domain, the discrete nature of graph topology makes the worst-case adversarial samples $S^{\prime}$ hard to be estimated.  
% All these issues, plus the non-i.i.d property of graph data, together pose a great challenge to the computation of GRV, which we aim to target in the next section.  
% \yang{check}
%Thus, the non-i.i.d and discrete nature of graph data makes the computation of GRV nontrival.  
% These challenges are 
% and more challenging compared with that in image domain.
% The non-i.i.d and discrete nature of graph data makes GRV  

% \begin{equation}
%     \text{GRV}_{\tau}(e) = \mathrm{I}\left((A, X) ; e\left((A, X)\right)\right) - \inf_{\mu_{(A^{\prime}, X^{\prime})} \sim \mathcal{B}_{\infty}(\mu_{(A, X)}, \tau)}  \mathrm{I}\left((A^{\prime}, X^{\prime}) ; e\left((A^{\prime}, X^{\prime})\right)\right)
% \end{equation}

% An end-to-end graph-based model $g$ is robust if it can function properly on a specific downstream task under adversarial perturbations. For \JR{unsupervised graph representation learning model $e$}, we argue that it is robust if it can capture the robustness of \JR{the encoder $e$} against input distribution perturbations in terms of mutual information between its input and output.

% A trust system is robust if it can function properly under
% all situations. For unfair rating attacks, we argue
% that a trust system is robust if it can function well under
% the worst case. To make a trust system robust to unfair
% rating attacks, we thus need to find the worst-case attacks
% first. The worst case then is: there is little information in recommendations, or misbehaving advisors try to minimise that information.

\subsection{Optimization Problem} \label{subsec:opt}

The trade-off between model robustness and the expressive power of encoder has been well-studied by many authors~\cite{tsipras2018robustness, zhang2019theoretically}.
In our case, this trade-off can be readily explored by the following optimization problem
\begin{equation} \label{eq:lb}
    % \mbox{maximize} \quad \ell_1(\Theta) =  \underbrace{\mathrm I(S;e(S))}_{\text {accuracy }} - \beta \underbrace{\mathrm{GRV}_\tau (e)}_{\text {robustness }},
    \mbox{maximize} \quad \ell_1(\Theta) = \mathrm I(S;e(S)) - \beta \mathrm{GRV}_\tau (e),
\end{equation}
where the optimization variable is the learnable parameters $\Theta$ of the encoder $e$, and $\beta > 0$ is a pre-defined parameter.

However, in practice, the ``most robust'' encoder is usually not the desired one (as it sacrifices too much in the encoder's expressive power).
An intuitive example for the ``most robust'' encoder is the constant map, which always outputs the same representation whatever the input is.
Hence, a ``robust enough'' encoder would be sufficient, or even better.
% \JR{explain more about the margin}
To this end, we add a soft-margin $\gamma$ to GRV,
and obtain the following optimization problem
\begin{equation} \label{eq:opt-prob}
    \mathrm{maximize} \quad \ell_2(\Theta) = \mathrm I(S;e(S)) - \beta \max {\{\mathrm{GRV}_\tau(e), \gamma\}}.
\end{equation}
The second term is positive if $\mathrm{GRV}_\tau > \gamma$ and the constant $\gamma$ otherwise.
As a result, when the encoder is sufficiently robust, the second term in~$\ell_2$ vanishes, and thus Problem~\eqref{eq:opt-prob} turns to the standard MI maximization using benign data.
% Under a mild assumption on $\beta$~\cite{BV04}, Problem~\eqref{eq:opt-prob} is equivalent to the constrained optimization problem
% \[
%     \begin{array}{ll}
%         \mbox{maximize} & \mathrm I(S;e(S)) \\
%         \mbox{subject to} & \mathrm{GRV}_\tau (e) \leq \gamma.
%     \end{array}
% \]
Furthermore, when $\beta=1$, Problem~\eqref{eq:opt-prob} can be divided into two simple sub-problems, depending on the value of $\mathrm{GRV}_\tau(e)$:
\begin{equation} \label{eq:obj}
    \left\{ \begin{aligned}
        &\max_{\Theta} \inf_{\mu_{S^{\prime}} \in \mathcal B_{\infty}(\mu_S, \tau)} \mathrm I (S^\prime; e(S^\prime)),  &&\text{if } \mathrm{GRV}_{\tau} 
        > \gamma \\
        &\max_{\Theta} \quad \mathrm I(S ; e(S)), &&\text{otherwise}.
    \end{aligned} \right.
\end{equation}
In this case ($\beta=1$), when $\mathrm{GRV}_\tau(e) > \gamma$, the problem maximizes the MI under the worst-case adversarial attack.
In other words, the robust encoder tries to maintain the mutual dependence between the graph data and the encoded representation, under all kinds of adversarial attacks. When the encoder is sufficiently robust (\emph{i.e.}, $\mathrm{GRV}_\tau (e) \leq \gamma$), the problem turns to maximize the expressive power of graph encoder.

\vpara{GNN as the parameterized encoder.}
The graph neural network (GNN) has been extensively used as an expressive function for parameterizing the graph encoder~\cite{kipf2016variational, kipf2017semi}.
In this paper, we adopt a one-layer GNN:
% the encoder architecture proposed in the seminal paper~\cite{kipf2017semi} which is a one-layer graph convolutional network (GCN):
% our encoder is a one-layer GNN that implements the following propagation rule:
% \[
%     e(\mathbf{A}, \mathbf{X})=\sigma(\hat{\mathbf{D}}^{-1/2} \hat{\mathbf{A}} \hat{\mathbf{D}}^{-1/2} \mathbf{X} \Theta),
% \]
$e(\mathbf{A}, \mathbf{X})=\sigma(\hat{\mathbf{D}}^{-1/2} \hat{\mathbf{A}} \hat{\mathbf{D}}^{-1/2} \mathbf{X} \Theta)$,
where $\hat{\mathbf A}$ is the adjacency matrix with self-loops, $\hat{\mathbf D}$ is the corresponding degree matrix, $\sigma$ is the ReLU function, and $\Theta$ is the learnable parameters.
% In line with these earlier works, we formulate our MI-based robust learning model as an optimization problem, considering the trade-off between the robustness and the representation capability of nature:
% % representation capability of nature and adversary:
% \begin{linenomath}
% \begin{align}
%  \mbox{\normalsize maximize}_{\Theta}  \quad  \ell_1(\Theta) \triangleq \mathrm{I}\left(S ; e\left(S\right)\right) - \beta\text{GRV}_{\tau}(e)  ,\label{eq:lb} 
% \end{align}
% \end{linenomath}
% where $\Theta$ represents the learnable parameter matrix of encoder $e_\Theta$ (we simplify $e_\Theta$ as $e$).

% \vpara{Robust training.}
% To ensure that our graph encoder is $(\tau, \gamma)$-robust, we investigate an alternative robust hinge loss. \JR{explain more about the margin} To achieve this end, we introduce a hinge loss penalty term to the standard formulation of $\text{GRV}_{\tau}(e)$ via the soft margin $\gamma$, and thus obtain the following objective:
% % We directly apply $\beta$ to replace $1-\beta$ in $\ell_2(\Theta)$ and thus obtain the objective:

% \begin{linenomath}
% \begin{equation*}
%     \ell_2(\Theta) = \mathrm{I}\left(S ; e\left(S\right)\right) - \beta \max(\text{RV}_{\tau}(e), \gamma).
% \end{equation*}
% \end{linenomath}

% The second term is positive if $\text{RV}_{\tau} \ge \gamma$ and zero otherwise; the model is robust with a margin of at most $\gamma$. In effect, if our model is sufficiently robust, the second term becomes zero, thus reducing $\ell_2(\Theta)$ to the standard mutual information maximization on natural (benign) examples with guaranteed robustness. It can be further cast as a saddle point problem by setting $\beta=1$ for simplicity in $\ell_2(\Theta)$, as follows:
% \begin{linenomath}
% \begin{equation}
% \label{eq:obj}
%     \left\{
%     \begin{aligned}
%         &\max_{\Theta} \min_{\mu_{S^{\prime}} \sim \mathcal{B}_{\infty}(\mu_{S}, \tau)} \mathrm{I}\left(S^{\prime} \text{;} e\left(S^{\prime}\right)\right), \  & \text{if } \text{RV}_{\tau} \ge \gamma\\
%         &\max_{\Theta} \quad \mathrm{I}\left(S ; e\left(S\right)\right), &\text{otherwise}.
%     \end{aligned}
%     \right.
% \end{equation}
% \end{linenomath}

% When $ \text{RV}_{\tau} \ge \gamma$, this objective function can be interpreted as an adversarial game between an adversary (who tries to find the worst-case adversarial distribution $\mu_{S^{\prime}}$) and a defender (who aims to protect the model from being attacked). 
% On the other hand, when the model is sufficiently robust (\emph{i.e.},  $ \text{RV}_{\tau} < \gamma$), we optimize the expressive power of the encoder $e$. 

% \vpara{GNNs for parameterizing encoder.}
% Commonly, graph neural networks (GNNs) take the graph topology and node attributes as inputs to learn node-level representations through the application of convolutional filters~\cite{wu2020comprehensive}.
% That being said, GNNs appear to be an expressive function for parameterizing the encoder $e$ given the graph-structured data.
% We here adopt the encoder architecture proposed in~\cite{velickovic2018deep}. More specifically, our encoder is a one-layer GNN that implements the following propagation rule~\cite{kipf2017semi}:
% $e(\mathbf{A}, \mathbf{X})=\sigma(\hat{\mathbf{D}}^{-1/2} \hat{\mathbf{A}} \hat{\mathbf{D}}^{-1/2} \mathbf{X} \Theta)$,
% where $\hat{\mathbf{A}}$ is the adjacency matrix with self-loops, $\hat{\mathbf{D}}$ is the corresponding degree matrix, $\sigma$ denotes the ReLU activation function, and $\Theta$ is the learnable weight matrix.


\hide{
\begin{equation} \label{eq:obj} \small
     \begin{array}{ll}
        \mbox{\normalsize maximize}_{\Theta} & \ell_1(\Theta) =  \mathrm{I}\left(S ; e\left(S\right)\right) \\
        \mbox{\normalsize subject to} & \text{RV}_{\tau}(e) \leq m,  \\
    \end{array}
\end{equation}

It has been demonstrated in recent works that robustness is at odds with the expressive power of graph encoder~\cite{tsipras2018robustness, zhang2019theoretically}. 
In line with these studies, we formulate our MI-based robust learning model as an optimization problem considering the trade-off between the representation capability of nature and adversary:
\begin{linenomath}
\begin{equation}
\text{maximize}_{\Theta} \quad \ell_1(\Theta) = \beta \mathrm{I}\left(S ; e\left(S\right)\right) + (1-\beta) \mathrm{I}\left(S^{\prime} ; e\left(S^{\prime}\right)\right), ~\label{eq:tradeoff}
\end{equation}
\end{linenomath}
where $\Theta$ represents the learnable parameter matrix of encoder $e_\Theta$ (we simplify $e_\Theta$ as $e$), $S= (A, X)$ is the random variable following the benign data distribution, and $S^{\prime}= (A^{\prime}, X^{\prime})$ denotes the variable following the adversarial distribution.

\vpara{A practically viable lower bound.}
To ensure the perturbations are imperceptible, the adversarial distribution $\mu_{S^{\prime}}$ is bounded in $\mathcal{B}_{\infty}(\mu_{S}, \tau)$. For a generic model, it is tricky to randomly select an adversarial distribution to compute $\mathrm{I}\left(S^{\prime} ; e\left(S^{\prime}\right)\right)$. Thereby, the problem of maximizing $\ell_1(\Theta) $, i.e., Problem~\eqref{eq:tradeoff}, can be properly relaxed to a problem of maximizing its lower bound $\ell_2(\Theta)$:
\begin{linenomath}
\begin{align}
   &\ell_1(\Theta) \ge 
   \beta \mathrm{I}\left(S ; e\left(S\right)\right) + (1-\beta) \inf_{\mu_{S^{\prime}} \sim \mathcal{B}_{\infty}(\mu_{S}, \tau)}  \mathrm{I}\left(S^{\prime} ; e(S^{\prime})\right) \nonumber \\
   & \qquad\ \;= \mathrm{I}\left(S ; e\left(S\right)\right) - (1-\beta)\text{RV}_{\tau}(e)  \triangleq \ell_2(\Theta) , \label{eq:lb} \\
    & \text{where} \ \text{RV}_{\tau}(e) = \mathrm{I}\left(S ; e\left(S\right)\right) - \inf_{\mu_{S^{\prime}} \sim \mathcal{B}_{\infty}(\mu_{S}, \tau)}  \mathrm{I}\left(S^{\prime} ; e\left(S^{\prime}\right)\right).  \nonumber
\end{align}
\end{linenomath}
The infimum in objective~\eqref{eq:lb} is attained to learn robust representations from the worst-case mutual information.
To take a close look at this formulation, we find that the representation vulnerability $\text{RV}_{\tau}(e)$ is exactly an extended version of the notion proposed by ~\cite{Zhu2020LearningAR} as a robustness measure of MI-based representation learning. A lower value of $\text{RV}_{\tau}(e)$ implies that the encoder is more robust to perturbations of input data distribution. Formally, a representation is deemed $(\tau, m)$-robust if $\text{RV}_{\tau}(e) \le m$.

\vpara{Robust training.}
To ensure our model is $(\tau, m)$-robust, we study an alternative robust hinge loss. To achieve this, we introduce a hinge loss penalty term to the standard formulation of $\text{RV}_{\tau}(e)$ via the soft margin $m$.
We directly apply $\beta$ to replace $1-\beta$ in $\ell_2(\Theta)$ and thus obtain the objective:
\begin{linenomath}
\begin{equation*}
    \ell_3(\Theta) = \mathrm{I}\left(S ; e\left(S\right)\right) - \beta \max(\text{RV}_{\tau}(e), m).
\end{equation*}
\end{linenomath}
The second term is positive if $\text{RV}_{\tau} \ge m$ and zero otherwise -- the model is robust with a margin of at most $m$. Effectively, if our model is sufficiently robust, the second term becomes zero, thus reducing $\ell_3(\Theta)$ to the standard MI maximization on natural (benign) examples with robustness guarantees.
It can be further cast into a saddle point problem by setting $\beta=1$ for simplicity in $\ell_3(\Theta)$, as follows:
\begin{linenomath}
\begin{equation}
\label{eq:obj}
    \left\{
    \begin{aligned}
        &\max_{\Theta} \min_{\mu_{S^{\prime}} \sim \mathcal{B}_{\infty}(\mu_{S}, \tau)} \mathrm{I}\left(S^{\prime} \text{;} e\left(S^{\prime}\right)\right), \  & \text{if } \text{RV}_{\tau} \ge m\\
        &\max_{\Theta} \quad \mathrm{I}\left(S ; e\left(S\right)\right), &\text{otherwise}.
    \end{aligned}
    \right.
\end{equation}
\end{linenomath}
When $ \text{RV}_{\tau} \ge m$, this objective function can be interpreted as an adversarial game between an adversary who tries to find the worst-case adversarial distribution $\mu_{S^{\prime}}$ and a defender who aims to protect the model from being attacked; one the other hand, when the model is robust enough (\emph{i.e.},  $ \text{RV}_{\tau} < m$), we turn to optimize the expressiveness of the encoder $e$.
}

\subsection{Approximate Solution} \label{subsec:solution}

In this section, we discuss in detail how to obtain a sub-optimal solution for Problem~\eqref{eq:obj}.
Overall, the algorithm we use is a variant of the classical gradient-based methods, as presented in Algorithm~\ref{alg:robust}.
In every iteration, we first find out the distribution of the worst-case adversarial attack, and thus we can calculate the value of $\mathrm{GRV}$.
If GRV is larger than $\gamma$, we try to enhance the robustness in this iteration, and apply one gradient descent step for the first sub-problem in Problem~\eqref{eq:obj}.
Otherwise when $\mathrm{GRV}_\tau(e) < \gamma$, the encoder is considered robust enough, and thus we focus on improving the expressive power by one gradient descent move in the second sub-problem in~\eqref{eq:obj}.
As a small clarification, the stopping criterion in Algorithm~\ref{alg:robust} follows the famous early-stopping technique~\cite{prechelt1998early}.

However, there are still many kinds of difficulties in implementing the algorithm.
First of all, the mutual information $\mathrm I(S, e(S))$ is extremely hard to compute, mainly because $S=(A,X)$ is a joint random variable involving a high-dimensional discrete variable $A$.
In addition, the search space of the adversarial attacks, $\mathcal B_\infty (\mu_S, \tau)$, is intractable to quantify:
There is no conventional or well-behaved choice for the distance metric $d$ in such a complicated joint space,
and even when we know the metric, the distance between two random variables is difficult to calculate.
Apart from the above challenges, the classical, well-known projected gradient descent algorithm does not work in the joint space $S=(A,X)$, and thus the worst-case adversarial attack $\mu_{S^\star}$ is no way to find.
Therefore, in this section, we further address the above issues in detail and explain every component in Algorithm~\ref{alg:robust}.

% As discussed above in Problem~\eqref{eq:obj}, we formulate the robust graph learning as two sub-problems and one of them is the saddle point optimization problem. 
% \JR{In this section, we first provide an optimization algorithm for Problem~\eqref{eq:obj}.
% Then, we provide a efficient and tractable solution to approximate it.}
% % a constrained saddle point optimization problem (as
% \yang{describe the major challenge of solving this optimization problem in one sentence} 

% \vpara{Framework for optimization.} \XJ{help to check}
% We hereby propose an optimization framework to solve Problem~\eqref{eq:obj}, which is shown in  Algorithm~\ref{alg:robust}, where the stopping criterion in the algorithm is a variant of early stopping~\cite{prechelt1998early}.
% First, we aim to find the worst-case adversarial distribution $\mu_{S^\star}$. Based on $\mu_{S^\star}$, $\text{GRV}_\tau$ can be computed.
% % randomly initialize the graph encoder parameters $\Theta$ (GNN as the instance). 
% % We then update $\Theta$ based on the objective of benign examples. 
% After that, according to the value of GRV, we alternately and iteratively update $\Theta$ based on the objective of the benign examples and that of the worst-case adversarial examples. 

% %\yang{Explain that MI and the infimum in Eq.~1 could not be calculated so far, which motivates the next section.} 

% However, mutual information remain intractable so far. 
% %If we are to solve the problem using an efficient gradient-based method, we should first estimate MI via neural networks, since direct computation would be intractable. 
% %(see the \textit{MI estimation} section for more details). 
% The other challenge is that of how to find the adversarial distribution $\mu_{S^{\prime}} \sim \mathcal{B}_{\infty}(\mu_{S}, \tau)$ in order to obtain the worst-case MI; to address this, we aim to choose an appropriate search space and efficiently find the adversarial perturbations.  
% %(see the \textit{Adversarial distribution estimation} section for more details). 
% We next introduce how to handle the above issues during optimization, under a graph transductive learning setting: all samples share the same  $\boldsymbol{s}=(\boldsymbol{a}, \boldsymbol{x})=(\mathbf{A}, \mathbf{X})$.

\begin{algorithm}[t]
\caption{Optimization algorithm. 
%Algorithm for Problem~\eqref{eq:obj}.
} \label{alg:robust}
	\begin{flushleft}
		\textbf{Input:} Graph $\mathbf{G}=(\mathbf{A}, \mathbf{X})$, learning rate $\alpha$. \\
		\textbf{Output:} Graph encoder parameters $\Theta$.
	\end{flushleft}
	\begin{algorithmic}[1]
		\STATE Randomly initialize $\Theta$.
		\WHILE {\textit{Stopping condition is not met}}
	        \STATE $\mu_{S^\star} \leftarrow  \mathop{\rm argmin}_{\mu_{S^\prime} \in \mathcal B(\mu_S, \tau)} \mathrm I(S^\prime; e(S^\prime))$.
	    
	        \STATE $\mathrm{GRV}_\tau (e) \leftarrow \mathrm I (S; e(S)) - \mathrm I(S^\star; e(S^\star))$.
		    \IF {$\mathrm{GRV}_\tau(e) > \gamma$}
    		    \STATE $\Theta \leftarrow \Theta - \alpha \nabla_\Theta  \mathrm{I} (S^\star; e(S^\star))$.
		    \ELSE
		        \STATE $\Theta \leftarrow \Theta - \alpha \nabla_\Theta \mathrm I(S; e(S))$.
		    \ENDIF
		\ENDWHILE
	\begin{flushleft}
		\textbf{Return:} $\Theta$.
	\end{flushleft}
	\end{algorithmic}
\end{algorithm}

\vpara{MI estimation.}
Directly computing $\mathrm I(S ; e(S))$ in Problem~\eqref{eq:obj} is intractable, especially for a joint distribution $S=(A,X)$ which includes a high-dimensional discrete random variable $A$.
Some authors propose to maximize the average MI between a high-level ``global'' representation and local regions of the input, and show great improvement in the quality of representations~\cite{hjelm2018learning, velickovic2018deep}.
Inspired by recent work Deep Graph Infomax~\cite{velickovic2018deep}, we use a noise-contrastive type objective as an approximation of the mutual information $\mathrm (I; e(S))$:
\begin{equation} \label{eq:jsd}
\ell_{\text{enc}}(S, e)
= \mathbb{E}_{S}\left[\log \mathcal{D}\left(\boldsymbol{z}, \boldsymbol{z}_{\mathbf{G}}\right)\right]  +  \mathbb{E}_{\tilde{S}}\left[\log \left(1-\mathcal{D}\left(\tilde{\boldsymbol{z}}, \boldsymbol{z}_{\mathbf{G}}\right)\right)\right],
\end{equation}
where $\boldsymbol{z}$ denotes the local representation; $\boldsymbol{z}_{\mathbf{G}} = \text{sigmoid}\left(\mathbb{E}_{S}(\boldsymbol{z})\right)$ represents the global representation; $\tilde{S}$ is the random variable of negative examples, and $\tilde{\boldsymbol{z}}$ represents the realization of $e(\tilde{S})$. 
The critic function $\mathcal{D}(\boldsymbol{z}, \boldsymbol{z}_{\mathbf{G}})$ represents the probability score assigned to a pair of local and global representations obtained from the natural samples (\emph{i.e.}, the original graph), while $\mathcal{D}(\tilde{\boldsymbol{z}}, \boldsymbol{z}_{\mathbf{G}})$ is that obtained from negative samples. 
Common choices for the critic function~$\mathcal{D}$ include bilinear critics, separable critics, concatenated critics, or even inner product critics~\cite{tschannen2019mutual}. 
Here, we select the learnable bilinear critic as our critic function; $\emph{i.e.}$, $\mathcal{D}_{\Phi} = \text{sigmoid}(\transpose{\boldsymbol{z}}\Phi\boldsymbol{z}_{\mathbf{G}})$, where $\Phi$ is a learnable scoring matrix.
Finally, in practice, the expectation over an underlying distribution is typically approximated by the expectation of the empirical distribution over $n$ independent samples $\{(\boldsymbol{a}^i, \boldsymbol{x}^i)\}_{i \in [n]}$.

\vpara{Adversarial distribution estimation.}
Besides the estimation of MI, another challenge involved in solving Problem~\eqref{eq:obj} is how to find the worst-case adversarial distribution $\mu_{S^{\prime}} \in \mathcal{B}_{\infty}(\mu_{S}, \tau)$. 
Here, we divide the difficulties in find $\mu_{S^\star}$ into three categories, and explain in detail how we solve them one by one.

First, it is difficult to choose an appropriate metric $d$ on the joint input space $\mathcal{S}=(\mathcal{A}, \mathcal{X})$ that faithfully measures the distance between each pair of point elements. 
For example, given any pair of points $\boldsymbol s_1 = (\boldsymbol a_1, \boldsymbol x_1)$ and $\boldsymbol s_2 = (\boldsymbol a_2, \boldsymbol x_2)$ in the joint metric space $(\mathcal A, d_\mathcal A)$ and $(\mathcal X, d_\mathcal X)$, an intuitive choice for the distance between $\boldsymbol s_1$ and $\boldsymbol s_2$ would be the $L_p$-norm $\|\big(d_{\mathcal{A}}(\boldsymbol a_1, \boldsymbol a_2), d_{\mathcal X}(\boldsymbol x_1, \boldsymbol x_2) \big)\|_p$.
However, this intuition fails in our case because the changes in graph topology and that in node attributes are not in the same order of magnitude.
Thereby, we have to consider the perturbations in $\mathcal A$ and $\mathcal X$ separately.
With a little abuse of notation, we redefine the perturbation bound as follows:
\begin{align*}
    \mathcal B_{\infty}(\mu_{A}, \mu_{X}, \delta, \epsilon) &= \{(\mu_{A^{\prime}},  \mu_{X^{\prime}}) \in \mathcal{M}(\mathcal{A}) \times \mathcal{M}(\mathcal{X}) \mid \\
    & W_{\infty}(\mu_{A}, \mu_{A^{\prime}}) \le \delta, W_{\infty}(\mu_{X}, \mu_{X^{\prime}}) \le \epsilon \},
\end{align*}
where the small positive numbers $\delta$ and $\epsilon$ play the role of perturbation budget now.
This is indeed a subset of the previous search space $\mathcal B(\mu_S, \tau)$.

% As is common, we can adopt the product metric to measure the Cartesian product $\mathcal{A} \times \mathcal{X}$ of two metric spaces $(\mathcal{A}, d_{\mathcal{A}})$ and  $(\mathcal{X}, d_{\mathcal{X}})$, \emph{i.e.}, $d = \| d_{\mathcal{A}}, d_{\mathcal{X}} \|_{p}$~\cite{deza2009encyclopedia}. More specifically, for any pair of points $(\boldsymbol{a}^1, \boldsymbol{x}^1), (\boldsymbol{a}^2, \boldsymbol{x}^2) \in \mathcal{S}$, the distance between them is calculated as $\| d_{\mathcal{A}}(\boldsymbol{a}^1, \boldsymbol{a}^2), d_{\mathcal{X}}(\boldsymbol{x}^1, \boldsymbol{x}^2) \|_{p}$.
% However, this approach fails in cases where our goal is to ensure imperceptible perturbations on $\mu_{A}$ and $\mu_{X}$ separately.
% Taking our case as an example, it is customary to limit the number of edge flips (\emph{i.e.}, $\ell_0$) so that it aligns with the discrete properties of the graph topology, while also limiting the $\ell_p$ norm of change in attributes, as is typically the case in the image domain.
% Note that the graph topology budget and node topology budget are not in the same order of magnitude; thus, we reduce the search space $\mathcal{B}_{\infty}(\mu_{S}, \tau)$ (where $d = \| d_{\mathcal{A}}, d_{\mathcal{X}} \|_{p}$ and $\tau = \|\delta, \epsilon \|_p$) to its subset so as to bring it into alignment with
% the adversarial setting on graphs, \emph{i.e.}, 
% \begin{linenomath}
% \begin{align*}
%     \mathcal{B}_{\infty}(\mu_{A}, \mu_{X}, \delta, \epsilon)=\{
%     &(\mu_{A^{\prime}},  \mu_{X^{\prime}}) \in \mathcal{M}(\mathcal{A}) \times \mathcal{M}(\mathcal{X}): \nonumber\\
%     W_{\infty}(&\mu_{A}, \mu_{A^{\prime}}) \le \delta, W_{\infty}(\mu_{X}, \mu_{X^{\prime}}) \le \epsilon \}. ~\label{eq:bound_two}
% \end{align*}
% \end{linenomath}
% Our goal is in fact to find a suboptimal solution in $\mathcal{B}_{\infty}(\mu_{S}, \tau)$.

Moreover, although the search space has been restricted, the $\infty$-Wasserstein constrained optimization problem remains intractable: We still have no clue about the underlying probability distribution.
Similar to what we did to estimate MI, we turn to replace the real data distribution with an empirical one.
Suppose we have a set of i.i.d. samples $\{(\boldsymbol a^i, \boldsymbol x^i)\}_{i \in [n]}$ (note that $n=1$ under a transductive learning setting, based on which we can compute the empirical distribution $(\hat \mu_A, \hat \mu_X)$).
The empirical search space
% $\hat{\mathcal B}(\{\boldsymbol a^i\}_{i=1}^n, \{\boldsymbol x^i\}_{i=1}^n, \delta, \epsilon)$
is defined as
\begin{align*}
    & \hat{\mathcal B} \big(\{\boldsymbol a^i\}_{i=1}^n, \{\boldsymbol x^i\}_{i=1}^n, \delta, \epsilon\big) \\
    &\qquad = \Big\{(\hat \mu_{A^\prime}, \hat \mu_{X^\prime}) \Bigm\vert \|{\boldsymbol a^i}^\prime - \boldsymbol a^i\|_0 \leq \delta, \|{\boldsymbol x^i}^\prime - \boldsymbol x^i\|_\infty \leq \epsilon, i \in [n] \Big\},
\end{align*}
where $\hat \mu_{A^\prime}$ and $\hat \mu_{X^\prime}$ are the empirical distributions computed from the perturbed samples $\{({{\boldsymbol a}^i}^\prime, {\boldsymbol x^i}^\prime)\}_{i \in [n]}$.
Here we use the cardinality (\emph{i.e.}, $L_0$-norm) to measure the change in graph topology (\emph{i.e.}, $\boldsymbol a$), and the $L_\infty$-norm to measure the change in continuous node attributes (\emph{i.e.}, $\boldsymbol x$).
(When node attributes are discrete, or even binary, we can also use $L_0$-norm for them.)
Finally, we notice that the empirical space $\hat{\mathcal B} \big(\{\boldsymbol a^i\}_{i=1}^n, \{\boldsymbol x^i\}_{i=1}^n, \delta, \epsilon\big)$ is again a subset of $\mathcal B_\infty(\hat \mu_A, \hat \mu_X, \delta, \epsilon)$.

% However, solving the $\infty$-Wasserstein  constrained optimization problem directly from the empirical distribution remains nontrival due to the non-linearity and the absence of duality of the $\infty$-Wasserstein distance~\cite{champion2008wasserstein}.
% We thus reduce the constraints w.r.t $\infty$-Wasserstein via $\mathcal{B}(\boldsymbol{a}, \boldsymbol{x}, \delta, \epsilon)$, and define the reduced search space as follows:
% \begin{linenomath}
% \begin{align*}
% &\mathcal{A}(\mathcal{C}, \delta, \epsilon)=\{(\hat{\mu}^{(n)}_{\{\boldsymbol{a}^{i\prime}\}_{i \in [n]}}, \hat{\mu}^{(n)}_{\{\boldsymbol{x}^{i\prime}\}_{i \in [n]}}): \\ 
% & \qquad\qquad\quad\ \ \ (\boldsymbol{a}^{i\prime}, \boldsymbol{x}^{i\prime}) \in \mathcal{B}(\boldsymbol{a}^i, \boldsymbol{x}^i, \delta, \epsilon)\ \ \forall i \in[n]\}, \\
% &\text{where } \hat{\mu}^{(n)}_{\{\boldsymbol{*}^{i\prime}\}_{i \in [n]}} = \frac1n  \sum_{i \in [n]}\mathbf{1}_{\{*^{i\prime}\}},
% \end{align*}
% \end{linenomath}
% where \JR{$\mathcal{C}=\{(\boldsymbol{a}^i, \boldsymbol{x}^i)\}_{i \in [n]}$ denotes the set of $n$ \emph{i.i.d.} samples (note that $n=1$ under a transductive learning setting)}, and $\mathbf{1}$ represents the indicator function (\emph{i.e.}, $\mathbf{1}_{\{*^{i\prime}\}}(x)=1$ if $x \in \{*^{i\prime}\}$ and $\mathbf{1}_{\{*^{i\prime}\}}(x)=0$ otherwise),
% and $\mathcal{B}(\boldsymbol{a}, \boldsymbol{x}, \delta, \epsilon) = \{ (\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}) \in \{0, 1\}^{|\mathbf{V}| \times |\mathbf{V}|} \times \mathbb{R}^{|\mathbf{V}| \times c}: \|\boldsymbol{a}^{\prime}-\boldsymbol{a}\|_0 \leq \delta , \|\boldsymbol{x}^{\prime}-\boldsymbol{x}\|_{\infty} \leq \epsilon\}$ is the empirical admissible perturbation bound around $\boldsymbol{a}$ and $\boldsymbol{x}$.
% Under the graph adversarial attack setting, we have $0 < \delta \ll |\mathbf{V}|^2$ as the budget constraint on the graph topology; furthermore, we use $\ell_0$ to measure the change in $\boldsymbol{a}$ due to its discrete nature. We also have $\epsilon \geq 0$ acting as the budget constraint on the node attributes, and use the $\ell_\infty$ norm to measure the change in $\boldsymbol{x}$ due to its continuous nature in most cases~\footnote{We can also use the $\ell_0$ to measure the change in $\boldsymbol{x}$ when the node attributes are discrete or binary in some cases.}.
% It can thus easily be shown that $\mathcal{A}(\mathcal{C}, \delta, \epsilon) \subseteq  \mathcal{B}_{\infty}(\hat{\mu}_{A}^{(n)}, \hat{\mu}_{X}^{(n)}, \delta, \epsilon)$.

The last, yet the most challenging difficulty is how to efficiently find the worst-case adversarial attack.
We know that he projected gradient descent (PGD) method can be used to find adversarial examples in the image domain~\cite{madry2017towards}.
However, the idea that works well for continuous optimization problems is not directly applicable in our case as the graph topology is a kind of Boolean variables.
Inspired by~\cite{xu2019topology},
as a remedy for the discrete case, we adopt a graph PGD attack for graph topology.
We first find a convex hull of the discrete feasible set, and apply the projected gradient method.
A binary sub-optimal solution $\boldsymbol a^\star$ is then recovered using random sampling.
This variant of PGD helps us identify the worst-case adversarial example efficiently.

% With the aid of first-order attack generation methods on images, it is easy to utilize the projected gradient descent method (PGD)~\cite{madry2017towards} to find the adversarial examples of $\boldsymbol{x}$ due to its continuous nature in most cases. However, it is not possible to directly apply continuous optimization methods to the graph topology, which is a kind of Boolean variable.
% As suggested in~\cite{xu2019topology}, we note that it is possible to project onto the feasible set defined by the convex hull of the Boolean variables. Accordingly, we adopt this type of projected gradient method on the graphs, then recover the binary worst-case solution of $\boldsymbol{a}$  via a randomization sampling approach. This kind of gradient-based method can help us efficiently identify the adversarial examples w.r.t the worst-case MI
% in Problem~\eqref{eq:obj}.

\hide{
As a result, we can obtain our approximate solution
of $\ell_3(\Theta)$:
\begin{linenomath}
\begin{equation}
\label{eq:finalobj}
    \left\{
    \begin{aligned}
        &\max_{\Theta, \Phi} \min_{\hat{\mu}^{(n)}_{S^{\prime}} \in \mathcal{A}(\mathcal{C}, \delta, \epsilon)}
        \ell_{\text{enc}}(S^{\prime}, e)
        % \mathrm{I}^{(\text{JSD})}\left(S^{\prime} \text{;} e\left(S^{\prime}\right)\right), 
        \  & \text{if } \widehat{\text{RV}}_{\tau} \ge \gamma\\
         &\max_{\Theta, \Phi} \quad 
        \ell_{\text{enc}}(S, e)
        %  \mathrm{I}^{(\text{JSD})}\left(S ; e\left(S\right)\right)
        , & \text{otherwise},
    \end{aligned}
    \right.
\end{equation}
\end{linenomath}
where $\widehat{\text{RV}}_{\tau}$ is the approximate value, while the parameters of the encoder $e$ (\emph{i.e.}, $\Theta$) and the parameters of the critic $\mathcal{D}$ (\emph{i.e.}, $\Phi$) are jointly optimized in the outer maximization step.
% The overall algorithm is presented in Algorithm~\ref{alg:robust}.
}

==> Robust unsupervised representation learning on graphs/prelim.tex <==
%!TEX root = robustgraph.tex

\section{Preliminaries and notations} \label{sec:pre}

In most cases, we use upper-case letters (\emph{e.g.}, $X$ and $Y$) to denote random variables and calligraphic letters (\emph{e.g.}, $\mathcal{X}$ and $\mathcal{Y}$) to denote their support, while the corresponding lower-case letters (\emph{e.g.}, $\boldsymbol{x}$ and $\boldsymbol{y}$) indicate the realizations of these variables. 
We denote the random variables of the probability distributions using  subscripts (\emph{e.g.}, $\mu_{X}$ and $\mu_{Y}$) and the corresponding empirical distributions with hat accents (\emph{e.g.}, $\hat{\mu}_{X}$ and $\hat{\mu}_{Y}$). We use bold upper-case letters to represent matrices (\emph{e.g.}, $\textbf{A}$). When indexing the matrices, $\textbf{A}_{ij}$ denotes the element at the $i$-th row and the $j$-th column, while $\textbf{A}_{i}$ represents the vector at the $i$-th row.
We use $(\mathcal{X}, d)$ to denote the metric space, where $d\, \text{:}\, \mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}$ is a distance function on $\mathcal{X}$.
% Let $\mathcal{B}(\boldsymbol{x}, \tau) = \{\boldsymbol{x}^\prime \in \mathcal{X}: d(\boldsymbol{x}^\prime, \boldsymbol{x}) \leq \tau \}$.
We further denote by $\mathcal{M}(\mathcal{X})$ the set of all probability measures on $\mathcal{X}$.

We assume a generic unsupervised graph representation learning setup. In brief, we are provided with an undirected and unweighted graph $\mathbf{G}=(\mathbf{V}, \mathbf{E})$ with the node set $\mathbf{V}= \{v_1, v_2, ..., v_{|\mathbf{V}|}\}$ and edge set $\mathbf{E} \subseteq  \mathbf{V} \times \mathbf{V} = \{e_1, e_2, ..., e_{|\mathbf{E}|}\}$. We are also provided with the adjacency matrix $\mathbf{A} \in \{ 0, 1\}^{|\mathbf{V}| \times |\mathbf{V}|}$ of the graph $\mathbf{G}$, a symmetric matrix with elements $\mathbf{A}_{ij}=1$ if $(v_i, v_j) \in \mathbf{E}$ or $i=j$, and $\mathbf{A}_{ij}=0$ otherwise. We augment $\mathbf{G}$ with the node attribute matrix $\mathbf{X} \in \mathbb{R}^{|\mathbf{V}| \times c}$ if nodes have attributes. Accordingly, we define our input as $\boldsymbol{s} = (\boldsymbol{a}, \boldsymbol{x}) \in \mathcal{S}$; thus, we can conceive of $\boldsymbol{x}$ as the attribute matrix and $\boldsymbol{a}$ as the adjacency matrix of $\mathbf{G}$ under a transductive learning setting, while $\boldsymbol{a}$ and $\boldsymbol{x}$ are the adjacency matrix and attribute matrix respectively of a node's subgraph under an inductive learning setting.
We further define an encoder $e: \mathcal{S} \rightarrow \mathcal{Z}$, which maps an input $\boldsymbol{s} = (\boldsymbol{a}, \boldsymbol{x}) \in \mathcal{S}$ to a representation $e(\boldsymbol{a}, \boldsymbol{x}) \in \mathcal{Z}$, and a simple machine learning model $f: \mathcal{Z} \rightarrow \mathcal{Y} $ that maps a representation $\boldsymbol{z} \in \mathcal{Z}$ to a label $f(\boldsymbol{z}) \in \mathcal{Y}$. 
We go on to define $g = f \circ e$ as their composition, such that $(f \circ e)(\boldsymbol{a}, \boldsymbol{x})=f(e(\boldsymbol{\boldsymbol{a}, \boldsymbol{x}}))$.
A table of main notations is attached in the Appendix.

\vpara{Mutual information.}
Recall that the mutual information between two random variables $X$ and $Y$ is a measure of the mutual dependence between them, and is defined as the Kullback--Leibler (KL) divergence between the joint distribution $p(\boldsymbol x, \boldsymbol y)$ and the product of the marginal distributions $p(\boldsymbol x) p(\boldsymbol y)$:
\begin{align*}
    \mathrm I (X; Y) 
    &= D_\mathrm{KL} \big(p(\boldsymbol x, \boldsymbol y) \| p(\boldsymbol x) p(\boldsymbol y) \big) \\
    &= \int_{\mathcal Y} \int_{\mathcal X} p(\boldsymbol x, \boldsymbol y) \log\left(\frac{p(\boldsymbol x, \boldsymbol y)}{p(\boldsymbol x) p(\boldsymbol y)}\right)  \, dx dy.
\end{align*}
More specifically, it quantifies the ``amount of information'' obtained about one random variable through observing the other random variable.
The successful application of mutual information to various unsupervised graph representation learning tasks has been demonstrated by many authors~\cite{velickovic2018deep, sun2019infograph, tschannen2019mutual}.

\vpara{Admissible perturbations on graphs.}
The Wasserstein distance 
%(a.k.a. the Earth mover's distance) 
can be conceptualized as an optimal transport problem: we wish to move transport the mass with probability distribution $\mu_S$ into another distribution $\mu_{S^\prime}$ at the minimum cost.
Formally, the $p$-th Wasserstein distance between 
%two probability measures 
$\mu_S$ and $\mu_{S^\prime}$ 
%in a metric space $(\mathcal S, d)$ 
is defined as
\[
    W_p = (\mu_S, \mu_{S^\prime}) = \left( \inf_{\pi \in \Pi (\mu_S, \mu_{S^\prime})} \int_{\mathcal S^2} d(\boldsymbol s, \boldsymbol s^\prime) \, d\pi(\boldsymbol s, \boldsymbol s^\prime) \right)^{1/p},
\]
where $\Pi(\mu_S, \mu_{S^\prime})$ denotes the collection of all measures on $\mathcal S \times \mathcal S$ with marginal $\mu_S$ and $\mu_{S^\prime}$, respectively.
The choice of $\infty$-Wasserstein distance (\emph{i.e.}, $p=\infty$) is conventional in learning graph representations~\cite{champion2008wasserstein}.

Based on $\infty$-Wasserstein distance, we can quantify the ability of the adversarial attacks.
An attack strategy is viewed as a perturbed probability distribution around that of $S=(A,X)$, and then all possible attack strategies stay in a ball around the genuine distribution~$\mu_S$:
\[
    \mathcal B_\infty(\mu_S, \tau) = \{\mu_{S^\prime} \in \mathcal M(S) \colon W_\infty (\mu_S, \mu_{S^\prime}) \leq \tau\},
\]
where $\tau > 0$ is a pre-defined budget.

% More specifically, consider the metric space $(\mathcal{S}, d)$; given two probability distributions $\mu_{S}$ and $\mu_{S^{\prime}}$ on the space, the $p$-th Wasserstein distance is defined as follows:
% \begin{linenomath}
% \begin{equation*}
%     W_p(\mu_{S}, \mu_{{S^{\prime}}})=\left(\inf_{ \pi \in \Pi(\mu_{S}, \mu_{S^{\prime}})} \langle \pi, d^p \rangle\right)^{1/p}
% \end{equation*}
% \end{linenomath}
% where $\langle \pi, d^p \rangle = \int_{\mathcal{S}^{2}} d(\boldsymbol{s}, \boldsymbol{s}^{\prime})^{p} \dif{\pi(\boldsymbol{s}, \boldsymbol{s}^{\prime})}$, while $\Pi(\mu_{S}, \mu_{S^{\prime}})$ denotes the set of all transportation plans over $\mathcal{S}^{2}$ with marginals $\mu_{S}$ and $\mu_{S^{\prime}}$ on the first and second factors, respectively. 
% We select the $\infty$-Wasserstein distance~\cite{champion2008wasserstein}--\emph{i.e.}, the limit of Wasserstein distance, as the measure of the two distributions throughout this work.
% \begin{linenomath}
% \begin{equation*}
%     \mathcal{B}_{\infty}(\mu_{S}, \tau)=\{\mu_{S^{\prime}} \in \mathcal{M}(\mathcal{S}): W_{\infty}(\mu_{S}, \mu_{S^{\prime}}) \le \tau \},
% \end{equation*}
% \end{linenomath}
% where $\mu_{S^{\prime}}$ denotes the adversarial distribution w.r.t $\mu_{S}$ here.


% \hide{
% some robustness measures built on the label space. The classification margin is commonly used to measure whether a node can be correctly classified, and has also been utilized to measure the robustness associated with GNNs~\cite{zugner2019certifiable, bojchevski2019certifiable}.
% \begin{definition} (Classification margin.)
% 	Let $y^{*}$ denote the ground truth class of the example $(\boldsymbol{a}, \boldsymbol{x})$; thus, the classification margin of $(\boldsymbol{a}, \boldsymbol{x})$ can be defined as:
% 	\begin{linenomath}
% 	\begin{equation*}
% 	%\mathbb{E}_{v \in 	\mathbf{V}} \left[ 
% 	\text{CM}(\boldsymbol{a}, \boldsymbol{x}, g, y^*) 
% 	= \max _{y \in  \mathcal{Y} \backslash \{y^*\}} \ln p(\hat{y} = y)
% 	-\ln p(\hat{y} = y^{*}), ~\label{def:margin}
% 	%\right]
% 	\end{equation*}
% 	\end{linenomath}
% \noindent where $\hat{y}=g(\boldsymbol{a}, \boldsymbol{x})$. 
% % The smaller the value of $\text{CM}(\boldsymbol{a}, \boldsymbol{x}, g, y^*)$, the more robust $g$ is w.r.t the example $(\boldsymbol{a}, \boldsymbol{x})$.
% \end{definition}
% \JR{do not emphasize CM, one definition of adversarial gap is enough}
% \YS{the above definition reads like it is a graph-level classification. }

% Building on the definition of the classification margin, we can define adversarial risk and adversarial gap, which measure the vulnerability of a given model under input perturbations on the joint input space~\cite{Zhu2020LearningAR}.
% \begin{definition}
% ~\label{def:ag}
% 	Let $(\mathcal{S}, d)$ denotes the input metric space and $y^{*}$ denote the ground truth class of the example $(\boldsymbol{a}, \boldsymbol{x})$. For any classification model $g: \mathcal{S} \rightarrow \mathcal{Y} $, we define the \textbf{adversarial risk} of $g$ with the adversarial budget $\tau \geq 0$ as follows:
% 	\begin{linenomath}
% 	\begin{equation*}\label{eq:advrisk}
% 		\begin{array}{ll}
% 			\text{AdvRisk}_{\tau}(g) = 
% 			& \mathbb{E}_{{p(\boldsymbol{s}, y^{*})}} 
% 			[
% 			\exists\  \boldsymbol{s}^{\prime}=(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}) \in \mathcal{B}(\boldsymbol{s}, \tau)  \\
% 			& \text { s.t. } 	\text{CM}(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}, g, y^*) \geq 0 ].
% 	    \end{array}
% 	\end{equation*}
% 	\end{linenomath}
% 	Based on $\text{AdvRisk}_{\tau}(g)$, the \textbf{adversarial gap} is defined to measure the relative vulnerability of a given model $g$ w.r.t $\tau$ as follows:
% 	\begin{linenomath}
% 	\begin{equation*}
% 	\text{AG}_{\tau}(g) = 	\text{AdvRisk}_{\tau}(g)  - \text{AdvRisk}_{0}(g).
% 	\end{equation*}
% 	\end{linenomath}
% \end{definition}
% }

==> Robust unsupervised representation learning on graphs/related.tex <==
%!TEX root = robustgraph.tex

\section{Related Works}
\label{sec:related}

\vpara{Unsupervised graph representation learning.}
The goal of unsupervised graph representation learning is to learn an encoder that maps the input graph into a low-dimensional representation space.
Currently, the most popular algorithms for unsupervised graph representation learning mainly rely on matrix factorization~\cite{von2007tutorial}, random walks~\cite{perozzi2014deepwalk, grover2016node2vec}, and adjacency matrix reconstruction~\cite{kipf2016variational, duran2017learning}. One alternative approach that has recently been advocated is that of adopting the MI maximization principle~\cite{linsker1988self,sun2019infograph, velickovic2018deep}. This type of methods have achieved massive gain in standard metrics across unsupervised representation learning on graphs, and is even competitive with supervised learning schemes. However, these MI-based graph embeddings usually do not perform well with noisy or adversarial data. This prompts further consideration of MI-based robust representation learning on graphs.

Additionally, there exist some unsupervised graph learning models targeting the adversarial vulnerability problem. One line of them tried to denoise the perturbed input based on certain hypothesis of the crafted attacks~\cite{entezari2020all, wu2019adversarial, dai2018adversarial}, such as the fact that  attackers tend to link two nodes with different features. Another trend focused on the robustness of a particular model, like Deepwalk~\cite{10.1145/3308558.3313445} and spectral clustering~\cite{bojchevski2017robust}.
However, most of them can only operate on certain task, but cannot be applied to various downstream tasks. 

\vpara{Robust models on graphs.}
% \JR{most robust models on graphs are supervised (e.g., GNN). when no label, gg. we focus on unsupervised encoder: mention SVD, RSC. introduce ours}
% Owing to the surge of adversarial attacks on graphs, several countermeasures have been proposed. 
Owing to the surge of adversarial attacks on graphs, several countermeasures have been proposed. Compared with pre/post-processing approaches, which are supported by empirical observations on specific attacks or models (mostly on GNNs), such as input denoising~\cite{wu2019adversarial, entezari2020all}, adversarial detection~\cite{bojchevski2017robust, xu2018characterizing, ioannidis2019graphsac} and certifiable robustness guarantees on GNNs~\cite{zugner2019certifiable, bojchevski2019certifiable, jin2020certified}, several recent attempts have been made to formulate the graph defense problem as a minimax adversarial game
~\cite{deng2019batch, feng2019graph, xu2019topology, chen2019can, wang2019graphdefense}. 
These approaches often resort to adversarial training for optimization due to its excellent performance; however, they typically require additional label information and are tailored to attacks on GNNs. 
On the other hand, another line of works that utilize a similar adversarial training strategy, do not depend on label information. For instance, one cheap method of this kind involves randomly dropping edges during adversarial training~\cite{dai2018adversarial}.
Moreover, in cases where no label information is exposed,
% so long as no label information is exposed,
there are some existing works~\cite{10.1145/3308558.3313445, yu2018learning} that have applied adversarial training to unsupervised representation learning (for example, DeepWalk and autoencoders).
However, the robustness of unsupervised representation learning via MI on graphs remains an inherent blind spot.

The work that most closely resembles ours is that of~\cite{Zhu2020LearningAR}, which develops a notion of representation vulnerability based on the worst-case MI in the image domain. 
However, it cannot address the robustness in the graph domain, mainly caused by 
%Unlike image domain,  a graph is a joint space $\mathcal S=(\mathcal A, \mathcal X)$ consisting of discrete graph topology and continuous node attributes. The 
the joint input space and the discrete nature of graph topology. 
%makes the representation vulnerability extremely difficult to estimate. 
Moreover, the adversarial perturbations of edges or node attributes are easy to propagate to other neighbors via the relational information on a graph, which makes the robustness even harder to enhance.
%We address these challenges in this paper.

% Our work focuses on the graph domain, where we have a joint input space of both graph topology and node attributes rather than a single input (e.g., image or graph topology only). A straightforward solution to extend Zhu, Zhang, and Evans 2020 to graph domain is to conduct robust representation learning on node attributes (X) and ignore graph topology (A). However, the existence of A breaks the i.i.d. assumption of X, leading to the robustness even harder to enhance because perturbations on A or X are easy to propagate to neighbors via relational information on a graph.
% As for our technique contribution, in the methodology level, we first propose a practical and explainable boundary to reduce the input search space. We then employ a perturbation strategy to target the discrete nature of A, which cannot be handled by Zhu, Zhang, and Evans 2020. In the theoretical level, we novelly establish a connection between model robustness and the robustness of downstream classiﬁers on graphs. The conclusions and assumptions are different with the theoretical analysis in Zhu, Zhang, and Evans 2020, as the distribution of representation is difficult to be derived due to the joint distribution of A and X as well as discrete data.
% In the end, comparing our work with the two papers mentioned by the reviewer, Zhu, Zhang, and Evans 2020 only studies in image domain; Veličković et al. 2019 never considers the robustness of learned representations.

% , where we have a joint input space of both graph topology and node attributes rather than a single input (e.g., image or graph topology only).

% Inspired by this work, we propose the graph representation vulnerability (GRV) and further demonstrate the theoretical connections between GRV and the robustness of downstream classifier under a joint input space.



==> Robust unsupervised representation learning on graphs/theory.tex <==
%!TEX root = robustgraph.tex

\section{Theoretical Connection to Label Space}
\label{sec:theory}

We expect our robust graph encoder is able to block perturbations on graphs and benefits the downstream tasks. To this end, in this section, we establish a provable connection between the robustness of representations (measured by our proposed GRV) and the robustness of the potential model built upon the representations.
% a clear connection with the potential model robustness of any classiﬁer that can be built upon a representation.
Despite the generalization of our framework, we take node classification tasks as an example in this section. 
First, we introduce a conventional robustness, adversarial gap (AG), to measure the robustness of downstream node classifier. Then, we explore some interesting theoretical connections between GRV and AG.

\vpara{Adversarial gap.} 
We here introduce a conventional robustness measure adversarial gap (AG) for node classification, which is built on the label space. 
\begin{definition}
~\label{def:ag}
Suppose we are under inductive learning setting, then $\boldsymbol{a}$ and $\boldsymbol{x}$ are the adjacency matrix and attribute matrix respectively of a node's subgraph.
Let $(\mathcal{S}, d)$ denote the input metric space and $\mathcal{Y} $ be the set of labels. %Let $p(\boldsymbol{s}, y^{*})$ be the joint distribution of the input and the ground truth class. 
% Suppose $\boldsymbol{s}=(\boldsymbol{a}, \boldsymbol{x})=(\mathbf{A}, \mathbf{X})$.
For node classification model $g: \mathcal{S} \rightarrow \mathcal{Y} $, we define the \textbf{adversarial risk} of $g$ with the adversarial budget $\tau \geq 0$ as follows:
	\begin{linenomath}
	\begin{equation*}\label{eq:advrisk}
		\begin{array}{ll}
			\text{AdvRisk}_{\tau}(g)
			&= 
			 \mathbb{E}_{{p(\boldsymbol{s}, y)}} 
			[
			\exists\  \boldsymbol{s}^{\prime}=(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}) \in \mathcal{B}(\boldsymbol{s}, \tau)  \\
			& \text { s.t. } g(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}) \not= y ]
% 			\text{CM}(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}, g, y^*) \geq 0 ].
	    \end{array}
	\end{equation*}
	\end{linenomath}
% 	\begin{linenomath}
% 	\begin{equation*}\label{eq:advrisk}
% 		\begin{array}{ll}
% 			\text{AdvRisk}_{\tau}(g)
% 			&= 
% 			 %\sum_{m=1}^{|\mathbf{V}|} 
% 			p[
% 			\exists\  \boldsymbol{s}^{\prime}=(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}) \in \mathcal{B}(\boldsymbol{s}, \tau)  \\
% 			& \text { s.t. } g(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime})_{m} \not= y_{m} ]
% % 			\text{AdvRisk}_{\tau}(g)
% % 			&= 
% % 			 \sum_{m=1}^{|\mathbf{V}|} 
% % 			p[
% % 			\exists\  \boldsymbol{s}^{\prime}=(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}) \in \mathcal{B}(\boldsymbol{s}, \tau)  \\
% % 			& \text { s.t. } g(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime})_{m} \not= y_{m} ]
% % 			\text{CM}(\boldsymbol{a}^{\prime}, \boldsymbol{x}^{\prime}, g, y^*) \geq 0 ].
% 	    \end{array}
% 	\end{equation*} 
% 	\end{linenomath}
	Based on $\text{AdvRisk}_{\tau}(g)$, the \textbf{adversarial gap} is defined to measure the relative vulnerability of a given model $g$ w.r.t $\tau$ as follows:
	\begin{linenomath}
	\begin{equation*}
	\text{AG}_{\tau}(g) = 	\text{AdvRisk}_{\tau}(g)  - \text{AdvRisk}_{0}(g).
	\end{equation*}
	\end{linenomath}
\end{definition}
The smaller the value of AdvRisk or AG is, the more robust $g$ is.

\hide{
\begin{definition}
Let $(\mathcal S, d)$ be the input space and $\mathcal Y$ the set of labels.
Suppose $p(s,y^\star)$ is the joint distribution of the input and the ground truth labels.
For any classification model $g \colon \mathcal S \to \mathcal Y$, we define the \textbf{adversarial risk} of $g$ with budget $\tau \geq 0$ as follows
\[
    \mathrm{AdvRisk}_\tau (g) = \mathbb E_{p(s,y^\star)} [s^\prime \mid s^\prime \in \mathcal E],
\]
where the set $\mathcal E$ contains all the adversarial attacks that successfully deceive the classification model $g$, i.e.,
\begin{align*}
    \mathcal E &= \Big\{s^\prime \Bigm\vert d(s^\prime, s) \leq \tau,
    \max_{y \in \mathcal Y \backslash \{y^\star\}} {\big(p(g(s^\prime)=y) - p(g(s^\prime)=y^\star)\big)} > 0 \Big\}.
\end{align*}
\end{definition}
}

%\YS{the above definition reads like it is a graph-level classification.}


\begin{table}[b]
\centering
\caption{Summary of robustness measures. %, which are defined based on the output space of $g$ or $e$. 
\small
Here, the adversarial gap ($\text{AG}$) 
%, Cf. Definition~\ref{def:ag}
is the robustness measure built on the label space $\mathcal{Y}$, while representation vulnerability ($\text{RV}$) and graph representation vulnerability ($\text{GRV}$) are MI-based measures built on the representation space $\mathcal{Z}$.
The subscript $\epsilon$ denotes the perturbation budget of $\boldsymbol{x}$ (\emph{i.e.}, the image) on the image domain, while the subscript $\tau$ denotes the perturbation budget of $(\boldsymbol{a}, \boldsymbol{x})$ on the graph domain. 
\normalsize
}
\begin{tabular}{p{2cm}<{\centering}p{1cm}<{\centering}p{2cm}<{\centering}p{1cm}<{\centering}}
\toprule
Robustness measure  &Domain & Input space                & Output space               \\\hline
$\text{AG}_{\epsilon}(g)$   &Image & Single $\mathcal{X}$                 & $\mathcal{Y}$ \\
$\text{AG}_{\tau}(g)$      &Graph  & Joint $(\mathcal{A}, \mathcal{X})$   & $\mathcal{Y}$ \\
$\text{RV}_{\epsilon}(e)$  &Image  & Single $\mathcal{X}$                 & $\mathcal{Z}$ \\
%  \cdashline{1-4}
$\text{GRV}_{\tau}(e)$      &Graph  & Joint $(\mathcal{A}, \mathcal{X})$   & $\mathcal{Z}$ \\
\bottomrule
\end{tabular}
\label{tab:robust}
\end{table}


Table~\ref{tab:robust} briefly summarize the robustness measures, including AG, RV and GRV.
% We start with a brief review of robustness measures in Table~\ref{tab:robust}.
%we can recall that 
% It's easy to see that 
The traditional model robustness, adversarial gap (\emph{i.e.}, $\text{AG}_{\epsilon}(g)$ and $\text{AG}_{\tau}(g)$), is based on the label space $\mathcal{Y}$, while the MI-based robustness measures (\emph{i.e.}, $\text{RV}_*(e)$ and $\text{GRV}_*(e)$) is built upon the representation space $\mathcal{Z}$.
The prior work~\cite{Zhu2020LearningAR}, which defines $\text{RV}_{\epsilon}(e)$ on a single input space $\mathcal{X}$ in the image domain has shown that $\text{RV}_{\epsilon}(e)$ has a clear connection with classifier robustness.
The graph representation venerability $\text{GRV}_{\tau}(e)$, however, defined as it is on a joint input space $(\mathcal{A}, \mathcal{X})$ in the graph domain, is different from images due to the existence of both discrete and continuous input data structures.
In what follows, we explore some interesting theoretic conclusions that an inherent relationship exists between the graph representation vulnerability  $\text{GRV}_{\tau}(e)$ and the adversarial gap $\text{AG}_{\tau}(g)$; this is based on some certain assumptions that is more aligned with the graph representation learning.

In exploring the GRV's connection to the label space $\mathcal{Y}$, one solution could be to simply assume that one of the input random variables (\emph{i.e.}, $A$ or $X$) and the label random variable $Y$ are independent. 
We first consider the two special cases as follows:
\begin{itemize}[]
\item Topology-aware: given $X \perp Y$, $p(Y|A,X) = p(Y|A)$
\item Attribute-aware: given $A \perp Y$, $p(Y|A,X) = p(Y|X)$
\end{itemize}

Here, we first work on these two special cases under the relevant assumptions. 
We then illustrate a more general case in which $Y$ is dependent on both $A$ and $X$.
Detailed proofs of the following theorems can be found in the Appendix.

\vpara{Special cases.}
% Recall that, in \S\ref{subsec:opt}, we adopt GNNs to parameterize the encoder $e$. 
% Here, we further 
We simplify the GNN-based encoder architecture as $\boldsymbol{z} = \transpose{\boldsymbol{a}} \boldsymbol{x}\boldsymbol{\Theta}$ to obtain a tractable surrogate model.
% so that we can obtain a tractable surrogate model. More specifically, we remove the nonlinearities of GNN following the method outlined in~\cite{wu2019simplifying}, including the last layer, and adopt one-layer GNN, leading us to obtain $\boldsymbol{z} = \transpose{\boldsymbol{a}} \boldsymbol{x}\boldsymbol{\Theta}$. 
% It is easy to show that the representation of each node depends only on its one-hop neighbors. Therefore, rather than operating with the adjacency matrix $\mathbf{A}$, we can obtain the corresponding column of $\mathbf{A}$ directly to compute the representation for each node. 
Thus, the representation of each node depends only on its one-hop neighbors, so we can obtain the corresponding column of $\mathbf{A}$ directly to compute the representation for each node. 
Additionally, inspired by~\cite{miyato2016adversarial, AdvT4NE_WWW2019} that have defined the perturbations on the intermediate representations, we opt to define the adversarial distribution w.r.t $\mu_{\transpose{A}X}$ instead of that w.r.t $\mu_{A}$ and $\mu_{X}$ respectively. This assumption is reasonable owing to our focus on the robustness of our model rather than the real attack strategies. Accordingly, we assume that the set of adversarial distributions is $\mathcal{B}_{\infty}(\mu_{\transpose{A}X}, \rho)=\{\mu_{\transpose{{A^{\prime}}}X^{\prime}} \in \mathcal{M}(\mathcal{H}):
W_{\infty}(\mu_{\transpose{A}X}, \mu_{\transpose{{A^{\prime}}}X^{\prime}}) \le \rho \}$  where $\mathcal{H} = \{\transpose{\boldsymbol{a}} \boldsymbol{x}: \forall \boldsymbol{a} \in \mathcal{A}, \boldsymbol{x} \in \mathcal{X} \}$ in the following two theorems.
% % Graph data is discrete, and the continuous adversarial noise can not be directly imposed on the discrete connected information
% \JR{Another modification is that we opt to define  the adversarial distribution w.r.t $\mu_{\transpose{A}X}$ instead. This assumption is also reasonable owing to our focus on the robustness of our model rather than the attack methods. Moreover, inspired by other works~\cite{miyato2016adversarial, AdvT4NE_WWW2019} that have defined the perturbations on the representation space, we use the assumption $W_{\infty}(\mu_{\transpose{A}X}, \mu_{\transpose{{A^{\prime}}}X^{\prime}}) \le \rho$ in two special theorems below.}

In Theorems~\ref{thm:att} and~\ref{thm:struct_i}, 
we use $\boldsymbol{a} \in \{0, 1\}^{|\mathbf{V}|}$ to denote a column of $\mathbf{A}$ and $\boldsymbol{x}=\mathbf{X}$. The subscript $\rho$ of GRV, AdvRisk and AG represents that they are defined via $\mathcal{B}_{\infty}(\mu_{\transpose{A}X}, \rho)$, while  $\mathcal{F}=\{f:z \mapsto y \}$ denotes the set of non-trivial downstream classifiers, $f^* = \arg \min_{f \in \mathcal{F}} \text{AdvRisk}_{\rho}(f \circ e)$ is the optimal classifier built upon $e$, and $H_b$ is the binary entropy function. 
Moreover, when indexing $\boldsymbol{a}$ and $\boldsymbol{x}$,  $\boldsymbol{a}_i$ denotes the $i$-th entry of $\boldsymbol{a}$ and $\boldsymbol{x}_i$ denotes the $i$-th row of $\boldsymbol{x}$.

\begin{theorem}[Topology-aware]~\label{thm:att}
Let $(\mathcal{A}, \|\cdot\|_{0})$ and $(\mathcal{X}, \|\cdot\|_{p})$ be the input metric spaces, $\mathcal{Y}=\{-1,+1\}$ be the label space and $\mathcal{Z} = \{-1, +1\}$ be the representation space. The set of encoders with $ \Theta \in \mathbb{R}^{|\mathbf{V}|}$ is as follows:
\begin{align}
% \[
\mathcal{E} = \{e: (\boldsymbol{a}, \boldsymbol{x}) \in \mathcal{S} \mapsto \operatorname{sgn}[\transpose{\boldsymbol{a}} \boldsymbol{x}\boldsymbol{\Theta}]|\  \| \boldsymbol{\Theta}\|_2 = 1\}.
% \]
~\label{eq:rep1}
\end{align}
Assume that all samples $(\boldsymbol{s}, \boldsymbol{y}) \sim \mu_{SY}$ are generated from $\boldsymbol{y} \stackrel{\text{u.a.r.}}{\sim} U\{-1, +1\}$, $\boldsymbol{a}_i \stackrel{\text{i.i.d.}}{\sim} \text{Bernoulli}(0.5 + \boldsymbol{y}\cdot (p - 0.5))$ and $\boldsymbol{x}_i \stackrel{\text{i.i.d.}}{\sim} \mathcal{N}(\boldsymbol{0}, \sigma^2 \boldsymbol{I}_c)$
where $i=1,2,\dots ,|\boldsymbol{V}|$ and $0 < p < 1$. Then, given $\rho \geq 0$, for any $e \in \mathcal{E}$, we have the following:
% \begin{linenomath}
% \begin{align}
\[
    \text{GRV}_{\rho}(e) = 1 - H_b(0.5 + \text{AG}_{\rho}(f^* \circ e)).
\]
% \end{align}
% \end{linenomath}
Next, consider a simpler case in which $\boldsymbol{y} \stackrel{\text{u.a.r.}}{\sim} U\{-1, +1\}$ and $\boldsymbol{a}_i \stackrel{\text{i.i.d.}}{\sim} \text{Bernoulli}(0.5 + \boldsymbol{y}\cdot (p - 0.5))$ hold, but $\boldsymbol{x}_i = \boldsymbol{1}_c,\ i=1,\dots ,|\boldsymbol{V}|$ and the set of encoders follows such that $\mathcal{E} = \{e : (\boldsymbol{a}, \boldsymbol{x}) \mapsto \operatorname{sgn}[(\transpose{\boldsymbol{a}} \boldsymbol{x} - 0.5|\boldsymbol{V}|\transpose{\boldsymbol{1}}_c) \boldsymbol{\Theta}]\ |\ \| \boldsymbol{\Theta}\|_2 = 1\}$,
% \begin{align*}
    % \mathcal{E} = \{e : (\boldsymbol{a}, \boldsymbol{x}) &\mapsto \operatorname{sgn}[(\transpose{\boldsymbol{a}} \boldsymbol{x} - 0.5|\boldsymbol{V}|\transpose{\boldsymbol{1}}_c) \boldsymbol{\Theta}]\ |\ \| \boldsymbol{\Theta}\|_2 = 1\},
% \end{align*}
which can be regarded as the non-attribute case.
Then, given $\rho \geq 0$, for any $e \in \mathcal{E}$, we have
\begin{linenomath}
\begin{align}
    1 - H_b(0.5 - 0.5 \text{AG}_{\rho}(f^* \circ e)) &\le \text{GRV}_{\rho}(e) \nonumber \\
    \le 1 - H_b(0.5 - &\text{AG}_{\rho}(f^* \circ e)). ~\label{ueq:rv1}
\end{align}
\end{linenomath}
\end{theorem}

Theorem~\ref{thm:att} reveals an explicit connection between  $\text{GRV}_{\rho}(e)$ and $\text{AG}_{\rho}(f^* \circ e)$ achieved by the best classifier in the topology-aware case.
We note that  $H_{b}(\theta)$ is concave on $(0,1)$ and that the maximum of $H_{b}$ is attained uniquely at $\theta=0.5$.
Thus, lower GRV is the sufficient and necessary condition of a smaller AG.

\begin{theorem}[Attribute-aware]~\label{thm:struct_i}
Let $(\mathcal{A}, \|\cdot\|_{0})$ and $(\mathcal{X}, \|\cdot\|_{p})$ be the input metric spaces, $\mathcal{Y}=\{-1,+1\}$ be the label space and $\mathcal{Z} = \{-1, +1\}$ be the representation space. Suppose that the set of encoders is as in ~\eqref{eq:rep1}.
Assume that the samples $(\boldsymbol{s}, \boldsymbol{y}) \sim \mu_{SY}$ are generated from $\boldsymbol{y} \stackrel{\text{u.a.r.}}{\sim} U\{-1, +1\}$, $\boldsymbol{a}_i \stackrel{i.i.d.}{\sim} \text{Bernoulli}(0.5)$ and $\boldsymbol{x}_i \stackrel{i.i.d.}{\sim} \mathcal{N}(\boldsymbol{y}\cdot \boldsymbol{\mu}, \sigma^2 I_c)$
where $i=1,2,\dots ,|\boldsymbol{V}|$. Then, given $\rho \geq 0$, for any $e \in \mathcal{E}$, we have:
\begin{linenomath}
\begin{equation}
    \text{GRV}_{\rho}(e) = 1 - H_b(0.5 - \text{AG}_{\rho}(f^* \circ e)).
\end{equation}
\end{linenomath}
Next, consider a simpler case in which $\boldsymbol{y} \stackrel{\text{u.a.r.}}{\sim} U\{-1, +1\}$, $\boldsymbol{x}_i \stackrel{i.i.d.}{\sim} \mathcal{N}(\boldsymbol{y}\cdot \boldsymbol{\mu}, \sigma^2 I_c)$  but $\boldsymbol{a} \in \{0, 1 \}^{|\boldsymbol{V}|}, \ \sum_{i=1}^{|\boldsymbol{V}|} \boldsymbol{a}_i = n_0 + n_1$, where $n_0 = |\boldsymbol{V}|/4 + \boldsymbol{y}\cdot (p - |\boldsymbol{V}|/4)$, $n_1 = |\boldsymbol{V}|/4 + \boldsymbol{y}\cdot (q - |\boldsymbol{V}|/4)$ and $p+q=|\boldsymbol{V}|/2, \ 0 \le p,q \le |\boldsymbol{V}|/2, \ p,q \in \mathbb{Z}$;
that is, $\transpose{\boldsymbol{a}}\boldsymbol{x}$ will aggregate $n_0$ samples with $\boldsymbol{y}=+1$ and $n_1$ samples with $\boldsymbol{y}=-1$. Further suppose that the set of encoders is as presented in \eqref{eq:rep1}. Then, given $\rho \geq 0$, ~\eqref{ueq:rv1} also holds for any $e \in \mathcal{E}$.
\end{theorem}
Similarly, we have $\text{GRV}_{\rho} \propto \text{AG}_{\rho}$ in  Theorem~\ref{thm:struct_i}.
% According to the attribute-aware case as in Theorem~\ref{thm:struct_i}, we can draw a similar conclusion as Theorem~\ref{thm:att}: \emph{i.e.}, $\text{GRV}_{\rho} \propto \text{AG}_{\rho}$.
Note that Theorems~\ref{thm:att} and \ref{thm:struct_i} still hold when $\boldsymbol{a}$ contains self-loops.
% In future work, we will address the case in which $Y$ is dependent on both $A$ and $X$, along with the connection to other downstream tasks.

\vpara{General case.} 
In the general case, we can extend~\cite[Theorem 3.4]{Zhu2020LearningAR} to the graph domain.
% by directly replacing the perturbation bound of distribution $\mu_{X}$ with that of the joint distribution $\mu_{AX}$ (\emph{i.e.}, $\mathcal{B}_{\infty}(\mu_{AX}, \tau)$).
Regardless of the encoder, the theorem below provides a general lower bound of adversarial risk over any downstream classifiers that involves both MI and GRV. We restate the theorem below.
\begin{theorem}\cite{Zhu2020LearningAR}.~\label{thm:gen}
Let $(\mathcal{S}, d)$ be the input metric space, $\mathcal{Z}$ be the representation space and $\mathcal{Y}$ be the label space. Assume that the distribution of labels $\mu_{Y}$ over $\mathcal{Y}$ is uniform and $S$ is the random variable following the joint distribution of inputs $\mu_{AX}$. Further suppose that $\mathcal{F}$ is the set of downstream classifiers. Given $\tau \ge 0$,
\begin{linenomath}
\begin{align*}
    \inf_{f \in \mathcal{F}} \text{AdvRisk}_{\tau}(f \circ e) \ge 1 - \frac{I(S;e(S))-\text{GRV}_{\tau}(e)+\log 2}{\log |\mathcal{Y}|}
\end{align*}
\end{linenomath}
holds for any encoder $e$.
\end{theorem}
Theorem~\ref{thm:gen} suggests that lower adversarial risk over all downstream classifiers cannot be achieved without either lower GRV or higher MI between $S$ and $e(S)$. It turns out that jointly optimizing the objective of maximizing $I(S;e(S))$ and that of minimizing $\text{GRV}_{\tau}(e)$ enables the learning of robust representations. Note that Theorem~\ref{thm:gen} also holds in the graph classification task.

==> impact.tex <==
%!TEX root = robustgraph.tex

\section{Ethics Statement}
\label{sec:impact}

Recently, deep learning on graphs has shown excellent results in different real-world applications including molecule analysis~\cite{hamilton2017inductive}, drug discovery~\cite{gilmer2017neural}, financial surveillance~\cite{paranjape2017motifs}, recommendation systems~\cite{wang2019knowledgeaware}, \emph{etc.}
Despite these impressive results, the research community has recently shown that graph learning models are vulnerable to adversarial attacks~\cite{chen2020survey, bojchevski2019adversarial, zugner2019adversarial}.
A graph attacker can intentionally modify the original graph such that the modifications are almost human-imperceptible, which can cause wrong predictions in graph learning models. The real-life applications of such attacks can be very serious, for instance, one could create some false connections with rich people to increase his/her credit score in an online payment company, then he/she will be able to get loan and run away from the system. 
For that reason, there is a pressing need to learn robust representations on graphs against these adversarial attacks.

In this paper, we focus on the underlying problem of learning robust representations via mutual information on graphs and further establish a theoretical connection between our robustness measure and the robustness of downstream classifiers. Our approach and analysis provide us some novel perspectives to better understand the vulnerability of graph learning models when facing with graph adversarial attacks.
Accordingly, we think our technology can bring beneficial impacts to the society. We would also encourage further works to develop better defense methods to maintain a more robust learning environment.
